Optimizing generalized Gini indices for fairness in rankings

There is growing interest in designing recommender systems that aim at being fair towards item producers or their least satisfied users. Inspired by the domain of inequality measurement in economics, this paper explores the use of generalized Gini welfare functions (GGFs) as a means to specify the normative criterion that recommender systems should optimize for. GGFs weight individuals depending on their ranks in the population, giving more weight to worse-off individuals to promote equality. Depending on these weights, GGFs minimize the Gini index of item exposure to promote equality between items, or focus on the performance on specific quantiles of least satisfied users. GGFs for ranking are challenging to optimize because they are non-differentiable. We resolve this challenge by leveraging tools from non-smooth optimization and projection operators used in differentiable sorting. We present experiments using real datasets with up to 15k users and items, which show that our approach obtains better trade-offs than the baselines on a variety of recommendation tasks and fairness criteria.

==> aliases.tex <==
\newcommand{\reals}{\mathbb{R}}

%%%%%%%%%%%%%%% stupid shortcuts

\newcommand{\lorenzeff}{Lorenz-optimality\xspace}


\newcommand{\myrescale}[2]{\scalebox{#1}{$\displaystyle #2$}}

\newcommand{\argmaxP}{\argmax_{\rrk\in\rrkS}}
\newcommand{\argmaxPl}{\argmax\limits_{\rrk\in\rrkS}}
\newcommand{\argmaxPls}{\smash{\argmax\limits_{\rrk\in\rrkS}}}
\newcommand{\argmaxU}{\argmax_{\bu\in\US}}
\newcommand{\argmaxUl}{\argmax\limits_{\bu\in\US}}
\newcommand{\argmaxUls}{\smash{\argmaxUl}}
\newcommand{\sumU}{\sum_{i\in\userS}}
\newcommand{\sumUl}{\sum\limits_{i\in\userS}}
\newcommand{\sumUls}{\smash{\sumUl}}
\newcommand{\sumI}{\sum_{j\in\itemS}}
\newcommand{\sumIl}{\sum\limits_{j\in\itemS}}
\newcommand{\sumIls}{\smash{\sumIl}}



\newcommand{\profileP}{\tuP}


%%%%%%%% for arrows
\usepackage{esvect} % better arrows
\RequirePackage{graphicx}
\RequirePackage{xparse}
\newcommand{\cvv}[1]{\reflectbox{\ensuremath{\vv{\reflectbox{\ensuremath{#1}}}}}} %inverted arrow
\NewDocumentCommand{\lN}{}{\mathpalette\dolN\relax} %inverted arrow keeping over math font size
\makeatletter
\NewDocumentCommand{\dolN}{mm}{%
  \reflectbox{\ensuremath{\vv{\reflectbox{\ensuremath{\m@th#1\mathcal{N}}}}}}%
}

%%%%%%%%%%% double arrow
\newcommand{\ifldr}{\reflectbox{\ensuremath{\fldr}}}
\newcommand{\symbrightftarrow}{\text{\smash{\raisebox{-.2ex}{%
    $\mkern4mu\fldr$}}}}
\newcommand{\symbleftarrow}{\text{\smash{\raisebox{-.45ex}{%
    $\ifldr\mkern4mu$}}}}
\newcommand{\accentrightarrow}[1]{\mathchoice
    {\accentset{\displaystyle\symbrightftarrow}{#1}}
    {\accentset{\textstyle\symbrightftarrow}{#1}}
    {\accentset{\scriptstyle\symbrightftarrow}{#1}}
    {\accentset{\scriptscriptstyle\symbrightftarrow}{#1}}
}
\newcommand{\accentleftarrow}[1]{\mathchoice
    {\accentset{\displaystyle\symbleftarrow}{#1}}
    {\accentset{\textstyle\symbleftarrow}{#1}}
    {\accentset{\scriptstyle\symbleftarrow}{#1}}
    {\accentset{\scriptscriptstyle\symbleftarrow}{#1}}
}
%\newcommand{\ccvv}[1]{\cvv{\vv{#1}}}
\newcommand{\ccvv}[1]{\accentleftarrow{\accentrightarrow{#1}}}

%%%%%%%%% modified transpose to be more beautiful with right arrows
\newcommand{\mytop}{{\text{\smash{\raisebox{.5ex}{$\mkern.4mu\top$}}}\!}}

%%%%%%%%% for hats in estimates
\RequirePackage{accents}
\DeclareMathSymbol{\widehatsym}{\mathord}{largesymbols}{"62}
\newcommand\lowerwidehatsym{%
  \text{\smash{\raisebox{-1.2ex}{%
    $\widehatsym$}}}}
\newcommand\fixwidehat[1]{%
  \mathchoice
    {\accentset{\displaystyle\lowerwidehatsym}{#1}}
    {\accentset{\textstyle\lowerwidehatsym}{#1}}
    {\accentset{\scriptstyle\lowerwidehatsym}{#1}}
    {\accentset{\scriptscriptstyle\lowerwidehatsym}{#1}}
}

\newcommand{\intint}[1]{[\![#1]\!]}
\newcommand{\grad}{\nabla}


\newcommand{\paretow}{\succeq_{\rm P}}
\newcommand{\lorenzw}{\succeq_{\rm L}}
\newcommand{\pareto}{\succ_{\rm P}}
\newcommand{\lorenz}{\succ_{\rm L}}

\newcommand{\rkS}{\mathfrak{S}}
\newcommand{\itemS}{{\intint{m}}}
\newcommand{\userS}{{\intint{n}}}

\newcommand{\n}{n}
\renewcommand{\ni}{{n_i}}
\renewcommand{\v}{v}
\newcommand{\nitems}{m}
\newcommand{\nusers}{n}
\newcommand{\edges}{\mathcal{E}}

\newcommand{\tmu}{\bar{\mu}}
\newcommand{\hmu}{\hat{\mu}}
\newcommand{\muij}{\mu_{ij}}
\newcommand{\hmuij}{\hmu_{ij}}
\newcommand{\hmuji}{\hmu_{ji}}
\newcommand{\muii}{\mu_{ii}}
%\newcommand{\uijprime}{\u_{ij'}}
\newcommand{\muji}{\mu_{ji}}
\newcommand{\mui}{\mu_{i}}
%\newcommand{\uj}{\u_{j}}
\newcommand{\tmuij}{\tilde{\mu}_{ij}}
\newcommand{\tmuijprime}{\tilde{\mu}_{ij'}}

\newcommand{\tempmu}{\tilde{\mu}}
\newcommand{\tempmuij}{\tempmu_{ij}}


\newcommand{\bw}{\xvector{w}}
\newcommand{\bu}{\xvector{u}}
\newcommand{\bup}{\xvector{u'}}
\newcommand{\bv}{\xvector{v}}
\newcommand{\bvp}{\xvector{v'}}
\newcommand{\bx}{\xvector{x}}
\newcommand{\bxm}{\overline{\bx}} % mean
\newcommand{\bxcum}{\xvector{X}}
\newcommand{\bycum}{\xvector{Y}}

\newcommand{\US}{\mathcal{U}}
\newcommand{\USutil}{{\cal U}^\util_\beta}
\newcommand{\USgqua}{{\cal U}^\gqua_\beta}
\newcommand{\USgpar}{{\cal U}^\expo_\beta}


\newcommand{\tUS}{\overline{{\cal U}}}
\newcommand{\bucum}{\xvector{U}} %{\xvector{\vv{u}}} %requires esvect
\newcommand{\bvcum}{\xvector{V}} %{\xvector{\vv{u}'}} %requires esvect



\newcommand{\bzcum}{\xvector{Z}}
\newcommand{\bzcump}{\xvector{Z'}}

\newcommand{\buusers}{{\bu}_{\userS}}
\newcommand{\buitems}{{\bu}_{\itemS}}
\newcommand{\bvusers}{{\bv}_{\userS}}
\newcommand{\bvitems}{{\bv}_{\itemS}}

\newcommand{\bwusers}{{\bw}^{\userS}}
\newcommand{\bwitems}{{\bw}^{\itemS}}
\newcommand{\blambdausers}{{\blambda}^{\userS}}
\newcommand{\blambdaitems}{{\blambda}^{\itemS}}

\newcommand{\bucumusers}{\boldsymbol{U}_{\userS}}
\newcommand{\bucumitems}{\boldsymbol{U}_{\itemS}}
% \newcommand{\bvusers}{\boldsymbol{u}'_{\userS}}
% \newcommand{\bvitems}{\boldsymbol{u}'_{\itemS}}




\newcommand{\balpha}{\xvector{\alpha}}
\newcommand{\blambda}{\xvector{\lambda}}
\newcommand{\btypes}{\xvector{t}}
\newcommand{\ntypes}{T}
\newcommand{\mytype}{\tau}
\newcommand{\lorenzwt}{\succeq_{{\rm L}, \btypes}}
\newcommand{\leximin}{\mathop{>}_{\rm lex}}
\newcommand{\leximinw}{\mathop{\geq}_{\rm lex}}

\newcommand{\geqinf}{\mathop{\geq}\limits_{\alpha\to-\infty}}


\newcommand{\W}{W}
\newcommand{\Wtheta}{W_{\theta}}
\newcommand{\WthetaP}{\W_\theta(\rrk)}
\newcommand{\Wthetau}{\W_\theta(\bu)}
\newcommand{\WthetauP}{\W_\theta(\tuP)}

\newcommand{\Walpha}{\W_{\alpha}}
\newcommand{\Walphalambda}{\W_{\lambda,\alpha}}
\newcommand{\oW}{\overline{W}}
\newcommand{\Phii}{\Phi_i}
\newcommand{\Phij}{\Phi_j}



\newcommand{\Ui}{\U_i}
\newcommand{\UiP}{\U_i(P)}
\newcommand{\Vj}{\V_j}
\newcommand{\VjP}{\V_j(\rrk)}
\newcommand{\Vi}{\V_i}
\newcommand{\ViP}{\V_i(\rrk)}
\newcommand{\Uover}{\overline{u}}
\newcommand{\Vover}{\overline{v}}


\newcommand{\other}{m}
\newcommand{\tUother}{\tU_{\other}}

\newcommand{\UuserP}{U(P)}
\newcommand{\UuseriP}{U_i(P)}
\newcommand{\UitemjP}{\Vj(P)}



\newcommand{\rrkS}{\mathcal{P}}
\newcommand{\rrk}{P}
\newcommand{\rrkijk}{P_{ijk}}
\newcommand{\rrki}{P_i}
\newcommand{\rrkij}{P_{ij}}
\newcommand{\rrkijprime}{P_{ij'}}
\newcommand{\rrkji}{P_{ji}}
\newcommand{\rrkjik}{P_{jik}}
\newcommand{\rrkt}{\rrk^{(t)}}
\newcommand{\rrktmo}{\rrk^{(t-1)}}
\newcommand{\rrktp}{\rrk^{(t+1)}}
\newcommand{\rrkopt}{P^*}
\newcommand{\rrkopti}{P^*_i}
\newcommand{\hrrk}{\hat{P}}


%%%%%%%%%%% revisiting the revisit of fairness of exposure

\newcommand{\util}{{\rm eq}}
\newcommand{\gqua}{{\rm qua}}

\newcommand{\Objutilbeta}{F_\beta}
\newcommand{\ObjutilbetaP}{\Objutilbeta(\rrk)}
\newcommand{\Objutilbetau}{\Objutilbeta(\bu)}
\newcommand{\ObjutilbetauP}{\Objutilbeta(\tuP)}


\newcommand{\Objgquabeta}{F^\gqua_\beta}
\newcommand{\ObjgquabetaP}{\Objgquabeta(\rrk)}
\newcommand{\Objgquabetau}{\Objgquabeta(\bu)}



\newcommand{\Pen}{D}
\newcommand{\Penp}{D'}
\newcommand{\PenP}{\Pen(\rrk)}
\newcommand{\Penu}{\Pen(\bu)}
\newcommand{\PenpP}{\Penp(\rrk)}
\newcommand{\Penpu}{\Penp(\bu)}
\newcommand{\Penqua}{D^{qua}}
\newcommand{\PenquaP}{\Penqua(\rrk)}
\newcommand{\Penquau}{\Penqua(\bu)}


\newcommand{\totexp}{E}
\newcommand{\gexpj}{e_j}
\newcommand{\gexpjprime}{e_{j'}}
\newcommand{\gexpjP}{e_j(\rrk)}
\newcommand{\quaj}{q_j}
\newcommand{\gexpjprimeP}{e_{j'}(\rrk)}
\newcommand{\quajprime}{q_{j'}}
\newcommand{\totqua}{Q}


%%%%%%%%%%%%% revisiting fairness of exposure

%% criteria names
\newcommand{\lexpo}{{\rm lexpo}}
\newcommand{\expo}{{\rm expo}}

\newcommand{\lexp}{{\rm lexpo}}
\newcommand{\lpar}{{\rm lpar}}
\newcommand{\lrel}{{\rm lrel}}
\newcommand{\lcont}{{\rm lcont}}
\newcommand{\gpar}{{\rm par}}
\newcommand{\gcont}{{\rm cont}}

%%




\newcommand{\tgtjexpo}{t^\expo_j}
\newcommand{\tgtjgpar}{t^\gpar_j}
\newcommand{\tgtjgqua}{t^\gqua_j}

\newcommand{\ObjexpobetaP}{F^{\expo, \beta}(\rrk)}
\newcommand{\ObjgparbetaP}{F^{\expo}_\beta(\rrk)}





%%%% utilities

%\newcommand{\tu}{\xvector{u}}
\newcommand{\htu}{\hat{\xvector{u}}}
\newcommand{\htui}{\hat{u}_i}

%\renewcommand{\u}{\xvector{u}}

\newcommand{\tuP}{\tu(\rrk)}
\newcommand{\tuPitems}{{\tu}_{\itemS}(\rrk)}
\newcommand{\tuitems}{{\tu}_{\itemS}}
\newcommand{\tuusers}{{\tu}_{\userS}}
\newcommand{\tuPusers}{{\tu}_{\userS}(\rrk)}


\newcommand{\tui}{\tu_i}
\newcommand{\tuj}{\tu_j}
\newcommand{\tujprime}{\tu_{j'}}
\newcommand{\tujP}{\tu_j(\rrk)}
\newcommand{\tujprimeP}{\tu_{j'}(\rrk)}
\newcommand{\tuiP}{\tu_i(\rrk)}
\newcommand{\tuiPopt}{\tu_i(\rrkopt)}



\newcommand{\tuopt}{\tu(\rrkopt)}
\newcommand{\tuexpo}{\tu^{\expo, \beta}}
\newcommand{\tuuv}{\tu^{\rm sum}}
\newcommand{\tuuvi}{\tu_i^{\rm sum}}
\newcommand{\tuuvitems}{\tu^{\rm sum}_{\itemS}}
\newcommand{\tuuvusers}{\tu^{\rm sum}_{\userS}}
\newcommand{\tutheta}{\tu^\theta}
\newcommand{\tuthetai}{\tu_i^\theta}
\newcommand{\tuthetausers}{\tu^\theta_\userS}
\newcommand{\tuthetaitems}{\tu^\theta_\itemS}
\newcommand{\tugqua}{\tu^{\gqua,\beta}}
\newcommand{\tugquai}{\tu_i^{\gqua,\beta}}
\newcommand{\tugquausers}{\tu^{\gqua, \beta}_\userS}
\newcommand{\tugquaitems}{\tu^{\gqua, \beta}_\itemS}
\newcommand{\tugquaprime}{\tu^{\gqua,\beta'}}
\newcommand{\tugpar}{\tu^{\expo,\beta}}
\newcommand{\tugpari}{\tu_i^{\expo,\beta}}
\newcommand{\tugparusers}{\tu^{\expo, \beta}_\userS}
\newcommand{\tugparitems}{\tu^{\expo, \beta}_\itemS}

\newcommand{\tuutil}{\tu^{\util, \beta}}
\newcommand{\tuutili}{\tu_i^{\util,\beta}}
\newcommand{\tuutilprime}{\tu^{\util,\beta'}}
\newcommand{\tuutilprimei}{\tu_i^{\util,\beta'}}
\newcommand{\tuutilusers}{{\tu}^{\util, \beta}_{\userS}}
\newcommand{\tuutilitems}{{\tu}^{\util, \beta}_{\itemS}}


\newcommand{\uuv}{\U^{\rm uv}}
\newcommand{\ugpar}{\U^{\gpar,\beta}}
\newcommand{\ugqua}{\U^{\gqua,\beta}}
\newcommand{\uuvi}{\U_i^{\rm uv}}
\newcommand{\ugpari}{\U_i^{\gpar,\beta}}
\newcommand{\ugquai}{\U_i^{\gqua,\beta}}
\newcommand{\ugparprime}{\U^{\gpar,\beta'}}
\newcommand{\ugquaprime}{\U^{\gqua,\beta'}}
\newcommand{\ugparprimei}{\U_i^{\gpar,\beta'}}
\newcommand{\ugquaprimei}{\U_i^{\gqua,\beta'}}



%%%%%%% experiments
\newcommand{\welf}{{\it welf}\xspace}
\newcommand{\patro}{{\it FairRec}\xspace}
\newcommand{\equalexpo}{{\it eq. exposure}\xspace}
\newcommand{\qualexpo}{{\it qua.-weighted}\xspace}
\newcommand{\equalu}{{\it eq. utility}\xspace}
\newcommand{\lastfmsmall}{Lastfm-2k\xspace}
\newcommand{\twitter}{Twitter-13k\xspace}





\newcommand{\conv}{{\rm conv}}
\newcommand{\wS}{{\mathcal{V}}}

\DeclareMathOperator{\prox}{prox}
%\DeclareMathOperator{\proj}{proj}
\DeclareMathOperator{\proj}{\Pi}
\DeclareMathOperator{\argsort}{argsort}

\newcommand{\ph}{\mathcal{C}} %permutahedron
\newcommand{\bc}{\xvector{c}} %generic vector c
\newcommand{\bcsig}{\xvector{c_\sigma}} %generic vector c permuted by \sigma
\newcommand{\by}{\xvector{y}}
\newcommand{\bz}{\xvector{z}}
\newcommand{\bzsig}{\xvector{z_\sigma}}
\newcommand{\bxsig}{\xvector{x_\sigma}}

\newcommand{\bwsig}{\xvector{w_\sigma}}
\newcommand{\bwsigt}{\xvector{w_\sigma^\intercal}}
\newcommand{\busig}{\xvector{u_\sigma}}
\newcommand{\tbw}{\xvector{\tilde{w}}}

\newcommand{\yt}{\xvector{y^{(t)}}}
\newcommand{\permSn}{\mathfrak{S}_n}

\newcommand{\PAV}{\texttt{PAV}\xspace}






%%%%%%% new commands by Virginie

\newcommand{\tu}{\xvector{\bar{u}}} % tmp: two-sided utility


\newcommand{\ubw}{\xvector{w^1}} % GGI weights for users
\newcommand{\ibw}{\xvector{w^2}} % GGI weights for items

\newcommand{\lw}{\xvector{w'}} % Lorenz weights
\newcommand{\ulw}{\xvector{w'^1}} % Lorenz weights for users
\newcommand{\ilw}{\xvector{w'^2}} % Lorenz weights for items

\newcommand{\iw}{\lambda} % item weight
\newcommand{\ggi}{G}
\newcommand{\gini}{\mathrm{Gini}} % Gini index
\newcommand{\welfgini}{W_{\mathrm{Gini}}} % Gini index

\newcommand{\welfobj}{F}
\newcommand{\welfobjuser}{g^{\rm user}}
\newcommand{\welfobjitem}{g^{\rm item}}
\newcommand{\giniwelf}[1]{g_{#1}}





\newcommand{\ew}{\xvector{b}} % exposure weights

\newcommand{\uutil}{\xvector{u}} % user utilities
\newcommand{\iutil}{\xvector{v}} % item utilities


\newcommand{\uGGF}{g_{\ubw}} % gini of users
\newcommand{\iGGF}{g_{\ibw}} % gini of items

\newcommand{\utbw}{\xvector{\tilde{w}^1}} % reversed GGI weights for users
\newcommand{\itbw}{\xvector{\tilde{w}^2}} % reversed GGI weights for items

\newcommand{\uyt}{\xvector{y^{1,(t)}}}
\newcommand{\iyt}{\xvector{y^{2,(t)}}}


\newcommand{\sm}{\beta} % smoothing parameter

\newcommand{\fbeta}{f^{\sm}}
\newcommand{\fbetat}{f^{\sm_t}}
\newcommand{\fbetatucbt}{f^{\sm_t}_{\hmut + \radt}}
\newcommand{\fbetatmu}{f^{\sm_t}_{\mu}}
\newcommand{\hbeta}{h^{\sm}}

\newcommand{\Qt}{Q^{(t)}}
\newcommand{\Qtp}{Q^{(t+1)}}
\newcommand{\Qtpopt}{Q^{(t+1)}_{*}}

\newcommand{\powt}{^{(t)}}
\newcommand{\powtp}{^{(t+1)}}

\newcommand{\radt}{\rho\powt} % confidence radius at time t
\newcommand{\radtj}{\radt_j} % confidence radius at time t for item j

\newcommand{\sumt}{\sum_{t'=1}^t}
\newcommand{\sumtau}{\sum_{t=1}^\tau}

\newcommand{\ct}{c\powt}
\newcommand{\ctj}{c\powt_j} % clicks

\newcommand{\sigmat}{\sigma\powt}
\newcommand{\sigmatj}{\sigmat(j)}

\newcommand{\hmut}{\hat{\mu}\powt}
\newcommand{\hmutj}{\hmut_j}
\newcommand{\ucbt}{\hat{U}\powt}
\newcommand{\ucbtjk}{\ucbt_{jk}}


\newcommand{\sort}{^\uparrow}
\newcommand{\descsort}{^\downarrow}
\newcommand{\bzsort}{\xvector{z\sort}}

\newcommand{\topk}{\mathop{\text{top-}K}}

\newcommand{\ceil}[1]{\lceil#1 \rceil}
\newcommand{\floor}[1]{\lfloor#1 \rfloor}

%%% Function to generate weights
\newcommand{\Gini}{\texttt{Gini}\xspace} % classic gini index
\newcommand{\geom}{\texttt{geometric}\xspace} % geometric weights
\newcommand{\quantile}{\texttt{quantile}\xspace}
\newcommand{\Bonfer}{\texttt{Bonferroni}\xspace}

\newcommand{\fwsmooth}{FW-smoothing\xspace}
\newcommand{\fwsubgrad}{FW-subgradient\xspace}


\newcommand{\projbetaP}{\xvector{y}}
\newcommand{\projbetaPi}{y_i}
\newcommand{\projbetaPj}{y_j}


\newcommand{\ggfobj}{F_{\lambda,\ubw,\ibw}}


==> sections/old/batch_nonsmooth_fw.tex <==

\newpage
\section{Batch optimization with nonsmooth Frank-Wolfe [2p / 5.5p]} \label{sec:batch-fw}

\virginie{too long, will be made shorter}

The contribution of this section is to provide a scalable method for OWA optimization, which is applicable to generalized Gini indices from welfare economics.

The standard approach to optimizing the OWA formulation of a multi-objective problem is to solve the equivalent linear program derived by \citep{ogryczak2003solving} (we remind this approach in App. \ref{app:owa}). Because the utilities depend on 3d-tensors $\rrk \in \rrkS$ in our case, the linear program has $O(n \cdot m^2)$ variables and constraints, which is prohibitively large in practice. 

On the other hand, the Frank-Wolfe algorithm \citep{frank1956algorithm} was previously used to optimize over global stochastic ranking, with provable computational efficiency and convergence guarantees \citep{do2021two}. However, it does not apply to GGFs, because sorting utilities makes OWAs non-differentiable. 

In this section, we build on the nonsmooth Frank-Wolfe method of \citep{nesterov2005smooth,lan2013complexity} and show how it can be leveraged for fast computation and convergence, when optimizing OWAs over global stochastic rankings. %It uses a smooth approximation of the GGF, for which we show that the gradient can be computed efficiently. We obtain provably fast computation and convergence in the case of OWA and rankings.
\nico{at this stage, maybe give the intuition of what remains to be done in addition of Lan}

\paragraph{Notation} $\norm{\bz}_p = \left(\sum_{i=1}^n (z_i)^p \right)^{\frac{1}{p}}$ denotes the $\ell_p$ norm, and when unambiguous, we use $\|\cdot \|$ as a shorthand for $\|\cdot \|_2$. Given a linear map $h,$ $\norm{h}$ denotes the operator norm of $h,$ and $h^*$ is its adjoint. The Euclidean projection onto a convex $\mathcal{C}$ is denoted by $\proj_{\mathcal{C}}(\bz):= \argmin\limits_{\bc \in \mathcal{C}} \frac{1}{2} \norm{\bz - \bc}^2.$ $D_\mathcal{C} = \max\limits_{\bx, \bx' \in \mathcal{C}}\|\bx - \bx'\|$ denotes the diameter of $\mathcal{C}.$


\subsection{Frank-Wolfe for Nonsmooth Problems}

For clarity, we present here the algorithm for the simpler objective of minimizing one GGF of user utilities $\uGGF(\bu(P))$, and later explain in Section \ref{sec:two-gini} how to easily use the algorithm to optimize a linear combination of two GGF, which is our main objective \eqref{eq:owaobj}. Let us fix the OWA weights $\ubw := \bw$ and denote the GGF $g(\bu(P)) := g_{\bw}(\bu(P))$. We also introduce $h(\bz) = -g(\bz)$ and $f(P) = h(\bu(P))$, to obtain a convex minimization problem: $\min\limits_{\rrk\in\rrkS} f(\rrk)$. We notice that $h$ is $\|\bw\|$-Lipschitz continuous, and that:
\begin{align}
    h(\bu(P)) = -\min_{\sigma \in \permSn} \bwsigt \bu(P) = \max_{\sigma \in \permSn } -\bwsigt \bu(P).
\end{align}
We consider the smooth approximation\footnote{It is also equal to the Moreau envelope of $h$, by strong duality.} of $h$ from \cite{nesterov2005smooth}, defined as: 
\begin{equation}
    \hbeta(\bz) = \max_{\by \in \reals^n} \xdp{\bz}{\by} - h^*(\by) - \frac{\beta}{2}\|\by\|,
\end{equation} for some smoothing parameter $\beta > 0$.  We denote $\fbeta(P) = \hbeta(\bu(P)).$ The proximal operator is defined as $\prox_{\phi}(\bz) = \argmin _{\bz' \in \mathcal{U}} \phi(\bz) + \frac{1}{2}\|\bz'-\bz\|^2.$

Our algorithm for minimizing $f$ is the nonsmooth Frank-Wolfe method from \citep{lan2013complexity} (Alg. \ref{alg:nonsmoothfw}, App. \ref{app:morealgo}) which constructs iterates $P^{(t)}$ at each iteration $t.$ Given a positive sequence $(\beta_t)_{t\geq 1}$ decreasing to $0$, at each iteration $t$, the algorithm takes a direction finding step with respect
to the smooth approximation $\fbetat$ of $f$, by calculating:
\begin{align}\label{eq:fw-step}
    &\Qt = \argmin_{\rrk\in\rrkS} \xdp{\rrk}{\grad \fbetat(P^{(t)}}).
\end{align}
The following lemma states previously established results on a formulation of $\grad \fbetat(P^{(t)}),$ as well as on the smoothness and approximation properties of Nesterov's smoothing (see e.g., \citet{yurtsever2018conditional,2020thekumparampil}).

\begin{lemma}[Useful properties of $\fbeta$]\label{lem:moreau} Let $\beta > 0.$
\begin{enumerate}
    \item Smoothness: $\fbeta$ is $\frac{\|\bu\|^2}{\beta}$-smooth and $\grad \fbeta(P) = \frac{1}{\beta} \bu^* (\bu(P) - \prox_{\beta h}(\bu(P)).$
    \item Error bound: $\forall \bz,\, \hbeta(\bz) \leq h(\bz) \leq \hbeta(\bz) + \frac{\beta}{2}\|\bw\|^2$.
\end{enumerate}
\end{lemma}

The parameter $\beta$ controls the trade-off between the smoothness of $\fbeta$ and the quality of its approximation of $f.$ The following convergence rate is obtained:

\begin{proposition}[Th. 4, \citet{lan2013complexity}]\label{prop:converge} With $\beta_0 = \frac{2 D_{\rrkS} \|\bu\|}{\|\bw\|} $, Algorithm \ref{alg:full} obtains the following convergence rate: $$f(P^{(T)}) - f(P^*) \leq \frac{2 D_{\rrkS} \|\bu\|\|\bw\|}{\sqrt{T+1}}.$$
\end{proposition}

\subsection{Efficient computation}

We now show how to compute step \eqref{eq:fw-step} efficiently.

\paragraph{Efficient computation of the Frank-Wolfe step} Frank-Wolfe methods shine when step \eqref{eq:fw-step} can be computed efficiently, which was shown to be the case for smooth ranking objectives \citep{do2021two}. In our case, the form of $\grad \fbeta(P)$ given by Lemma \ref{lem:moreau} as a function of $\bu^*$ enables to solve step \eqref{eq:fw-step}  with only one top-$K$ sorting operation per user. Indeed, let $\topk(\bz) = \{ \sigma \in \permSn: z_{\sigma(1)}\geq \ldots \geq z_{\sigma(K)}\}$. When given access to $\prox_{\beta h}(\bu(P))$, we have:

\begin{proposition}[Th. 1, \citet{do2021two}]\label{prop:fwgrad}
Let $\yt = \frac{1}{\beta_t}(\bu(P^{(t)})- \prox_{\beta_t h}(\bu(P^{(t)}))$ and $\tempmuij = \yt_i \muij$. For all $i \in \intint{n},$ let $\tilde{\sigma}_i \in \topk(\tilde{\mu}_i)$ and $\Qt_i$ a permutation matrix representing $\tilde{\sigma}_i$.
Then $\Qt \in \argmin\limits_{\rrk \in \rrkS} \xdp{\rrk}{\grad \fbetat(\rrkt)}.$
\end{proposition}


\paragraph{Efficient computation of $\protect\prox_{\beta h}(\protect\bu(P))$} The main challenge of using Nesterov's smoothing is the calculation of $\prox_{\beta h}(\bv),$ on which relies the direction finding step \eqref{eq:fw-step}. We show that in our case, $\prox_{\beta h}(\bv)$ can be computed efficiently using a reduction to isotonic regression.

For $\bz \in \reals^n$, let $\ph(\bz)$ denote the permutahedron induced by $\bz$, defined as the convex hull of all permutations of the vector $\bz$: $\,\ph(\bz) = \conv\{\bcsig : \sigma \in \permSn\}.\,$ Then $h$ can be written as the support function of the convex $\ph(\tbw)$, where $\tbw = -(w_n,...,w_1)$:
\begin{align*}
    h(\bz) = \max_{\sigma \in \permSn} -\bwsigt \bz = \sup_{\by \in \ph(\tbw)} \by^\intercal \bz.
\end{align*}
Then the conjugate of $h$ is known to be the indicator function of the convex $\ph(\tbw)$, and its proximal is the projection $\proj_{\ph(\tbw)}$ \citep{parikh2014proximal}. By Moreau decomposition, we get: $~\prox_{\beta h}(\bz) = \bz - \beta \proj_{\ph(\tbw)}\left(\nicefrac{\bz}{\beta}\right),$ and thus:
\begin{equation}
\begin{aligned}\label{eq:yt-proj}
    \yt =  \proj_{\ph(\tbw)}\left(\frac{\bu(\rrkt)}{\sm_t}\right)
\end{aligned}
\end{equation}


Therefore, computing $\prox_{\beta h}$ and the $\yt$ of Proposition \ref{prop:fwgrad} boils down to a projection onto the permutahedron $\ph(\tbw)$. This projection was shown by several authors to be reducible to isotonic regression \citep{negrinho2014orbit,lim2016efficient,blondel2020fast}.

\begin{proposition}[Reduction to isotonic regression]\label{prop:isoto} Let $\sigma\in\permSn$ that sorts $\bz$ decreasingly, i.e. $z_{\sigma(1)} \geq \ldots \geq z_{\sigma(n)}.$
Let $\bx$ be a solution to isotonic regression on $\bzsig - \bw$, i.e.
\begin{align}
    \bx = \argmin_{x'_1 \leq \ldots \leq x'_n} \frac{1}{2}\|\bx' - (\bzsig - \bw)\|^2
\end{align}
Then we have: $ \proj_{\ph(\tbw)}(\bz) = \bz + \xvector{x_{\sigma^{-1}}}.$
\end{proposition}


We use the Pool Adjacent Violators (\PAV) algorithm for isotonic regression, which was shown to output an exact solution in $O(n)$ iterations given a sorted input \cite{best2000minimizing}. Including the sorting of the input, the routine for computing $\yt$ only costs $O(n \log n)$ time and $O(n)$ space. 

The computation of the direction step \eqref{eq:fw-step}, summarized in Alg. \ref{alg:fwsmooth-step}, is the main contribution of our approach. %The full nonsmooth Frank-Wolfe algorithm for ranking is described in Alg. \ref{alg:full}, App. \ref{app:morealgo}.
\virginie{insist before that this module is the main contribution, and a flexible approach we can use in the bandit setting later too}

% \paragraph{Summary of step \eqref{eq:fw-step}} Using \eqref{eq:prox}, the vector $\yt$ of Proposition \ref{prop:fwgrad} simply writes as the projection
% \begin{equation}
% \begin{aligned}
%     \yt =  \proj_{\ph(\tbw)}\left(\frac{\bu(\rrkt)}{\sm_t}\right),
% \end{aligned}
% \end{equation}
% and is computed by the formula of Proposition \ref{prop:isoto} using the Pool Adjacent Violators algorithm. The solution of step \eqref{eq:fw-step} is then obtained as a $\topk(\yt_i\mu_i)$ for each user $i$. Our full algorithm is described in Alg. \ref{alg:full}, App. \ref{app:morealgo}.


\paragraph{Complexity} Putting the results of Propositions \ref{prop:fwgrad} and \ref{prop:isoto} together, we obtain the following complexity result:

\begin{proposition}\label{prop:complexity} With $\beta_0 = \frac{2 D_{\rrkS} \|\bu\|}{\|\bw\|} $ and $(\beta_t)_{t} = \left(\frac{\beta_0}{\sqrt{t+1}}\right)$, Alg. \ref{alg:fwsmooth-step} runs with $O(n \ln n + m \ln K)$ operations per user and requires $O(n + K)$ memory.
\end{proposition}
\nico{it feels like the memory requirement is a bit unclear -- in welf the phrasing is ``Moreover, for each user, an iteration costs $O(\nitems\ln K)$ operations and requires $O(K)$ additional bytes of storage.''. It's not super clear tht if you want the actual solution, you neet $O(n K \# iterations)$ of storage.}
Moreover, the algorithm provides a sparse representation of the stochastic rankings as a weighted sum of permutation matrices. In other words, this gives us a Birkhoff-von-Neumann decomposition for free, without having to use additional polynomial time \nico{you seem to use ``polynomial time'' as if it was a bad thing :D} \virginie{whoops}algorithms to sample rankings as in previous work \citep{singh2018fairness}. 



\begin{algorithm}\label{alg:fwsmooth-step}
    \caption{Frank-Wolfe direction step \eqref{eq:fw-step}}
    \DontPrintSemicolon
     \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
     
     \Input{utilities $\bu(\rrkt)$, smoothing $\sm_t$, weights $\bw$}
     \Output{deterministic ranking $\Qt$}
     $\sigma \gets \argsort\descsort(\frac{\bu(P^{(t)})}{\beta_t})$ and  $\bz \gets \frac{\bu(P^{(t)})}{\beta_t}$\;
     $\bx \gets \PAV(\bzsig - \bw)$\;
     $\yt \gets \bz + \xvector{x_{\sigma^{-1}}}$\;
     \lFor{i=1, \ldots, \n}{
         $\tilde{\mu}_i \gets \yt_i \mui~$ and $~~\tilde{\sigma}_i \gets \topk( \tilde{\mu}_i )$} Return $\Qt \in \rrkS$ such that $\Qt_i$ represents  $\tilde{\sigma}_i$.\;
\end{algorithm}

\

\subsection{Two-sided fairness objective} \label{sec:two-gini}

Our objective \eqref{eq:owaobj} is $F(P) = G(
\bu(P),\bv(P))$, which is a linear combination of two GGFs, $\uGGF(\bu(\rrk))$ and $\iGGF(\bv(\rrk))$. 
Since $G$ is a separable sum, we have for $(\bx,\bx') \in \US$,
\begin{align*}
    \prox_{-\beta G}({\bx}^1,{\bx}^2) = \big(\prox_{-\beta \iw \uGGF}({\bx}^1), \prox_{-\beta (1-\iw)\iGGF}({\bx}^2)\big),
\end{align*}
where $\prox_{-\beta \iw \uGGF}(\bx) = \bx - \iw \beta  \proj_{\ph({\utbw})}\left(\frac{\bx}{\iw \beta}\right)$ and similarly for $\prox_{-\beta (1-\iw)\iGGF}(\bx)$.

% \begin{equation}
%     \begin{aligned}
%         \prox_{\beta g_{\userS}}(\bvusers) = \bvusers - \beta \proj_{\ph({\tbw}_{\userS})}\left(\frac{\bvusers}{\beta}\right) \quad \text{ and } \quad         \prox_{\beta g_{\itemS}}(\bvitems) = \bvitems - \beta \proj_{\ph({\tbw}_{\itemS})}\left(\frac{\bvitems}{\beta}\right).
% \end{aligned}
% \end{equation}



Let $t\geq 0$ and $\yt=(\uyt, \iyt)~~$ such that $\uyt=\proj_{\ph({\utbw})}\left(\frac{\bu(\rrkt)}{\iw \sm_t}\right)$ and $\iyt=\proj_{\ph({\itbw})}\left(\frac{\bv(\rrkt)}{(1-\iw)\sm_t}\right).$ Let $\tempmuij = \iw \uyt_i \muij + (1-\iw)\iyt_j.$

Then we can adapt Algorithm \ref{alg:fwsmooth-step} to the minimization of the two-sided objective $-F$ with the following routine:
\begin{enumerate}
    \item Use Lines 1-2-3 twice to compute $\uyt$ and $\iyt$,
    \item Assign $\tempmuij \gets \iw \uyt_i \muij + (1-\iw)\iyt_j$ in Line 4.
\end{enumerate}

\begin{corollary}
The routine described above obtains the same convergence guarantee as Proposition \eqref{prop:converge} and computational complexity as Proposition \eqref{prop:complexity}.
\end{corollary}

\virginie{check the $\iw$ and if there are no additional constants for \eqref{prop:converge}. or simpler alternative: smooth each part separately with $\beta_0 = \frac{D_{\mathcal{P}}\norm{u}}{\norm{w}}$}


\subsection{Regret bound when preferences are estimated}

In practice, inference is carried out on an estimate $\hmu$ of $\mu$, meaning that, denoting $\htu$ the resulting estimated utility\footnote{We have $\htu_i(\rrk)=\sumI \hmu_{ij}\rrkij\ew$ for $i\in\userS.$} the system output $\hrrk = \argmaxP G(\htu(\rrk),\bv(\rrk))$. 
The following result extends surrogate regret bounds that exist in classification \citep{bartlett2006convexity,zhang2004statistical} and learning-to-rank \citep{cossock2008statistical,ravikumar2011ndcg,agarwal2014surrogate,kotlowski2011bipartite} 
to the case of OWAs and global stochastic rankings. It makes the link between the quality of the estimate $\hmu$ and an optimality guarantee for $F(\hrrk)$ (i.e., the true GGF of the ranking inferred on the estimated values).\
\begin{theorem}\label{thm:regretbound}
Let $(\hmu_{ij})_{i,j}$, $\hrrk = \argmax\limits_{\rrk\in\rrkS} G(\htu(\rrk),\bv(\rrk))$, and $\rrkopt = \argmax\limits_{\rrk\in\rrkS}F(P)$. We have:\begin{align}
    F(\rrkopt) - F(\hrrk) \leq 4\sqrt{n\norm{\ew}_2^2}
    %\smash{
    \sqrt{\sum_{1\leq i\leq n\atop 1\leq j \leq m}(\hmuij-\muij)^2}.
    %}
\end{align}
\end{theorem}
\virginie{todo: check proof for 2 gini}\nico{Is that true? I would say it is, since iirc the proof we had in the paper only requires subderivatives, but I'm not sure how you can ``prove'' that without a lengthy appendix.}

==> sections/old/experiments.tex <==
\section{Experiments} \label{sec:xps}

We first present our experimental setting for one-sided recommendation of movies and music, including a description of the competing fairness objectives we compare our GGF approach to. Then, we demonstrate the effectiveness of \fwsmooth compared to the simpler baseline of Frank-Wolfe with a subgradient (Sec. \ref{sec:xp-convergence}). In Sec. \ref{sec:xp-onesided-tradeoff}, we showcase the generality of GGF as a method to meet a large variety of fairness criteria in one-sided recommendation. Finally, in Sec. \ref{sec:xp-reciprocal}, we show similar benefits in reciprocal recommendation.

\subsection{Experimental setup} \label{sec:xp-setup}

Our experiments are implemented in Python 3.9 using PyTorch\footnote{\url{http://pytorch.org}}. For the \PAV algorithm, we use the implementation of Scikit-Learn.\footnote{\url{https://github.com/scikit-learn/scikit-learn/blob/main/sklearn/isotonic.py}}

\subsubsection{Data and evaluation protocol} 

We present experiments on two recommendation tasks. First, we address music recommendation with the \textbf{Lastfm-2k} from \citet{Cantador:RecSys2011} which contains real listening counts of $2k$
users for $19k$ artists on the online music service Last.fm\footnote{\url{https://www.last.fm/}}. We filter the $2,500$ items having the most listeners. In order to show how the algorithm scales, we also consider the \textbf{MovieLens-20m} dataset \cite{harper2015movielens}, which contains ratings in $[0.5,5]$ of movies by users, and we select the top $15,000$ users and items with the most interactions. 

We use an evaluation protocol similar to \cite{patro2020fairrec,do2021two,wang2020fairness}. For each dataset, a full user-item preference matrix $(\mu_{i,j})_{i,j}$ is obtained by standard matrix factorization algorithms\footnote{Using the Python library Implicit: \url{https://github.com/benfred/implicit} (MIT License).} from the incomplete interaction matrix. Rankings are inferred from these estimated preferences. The exposure weights $\ew$ are the standard weights of the \emph{discounted cumulative gain} (DCG) (also used in e.g., \cite{singh2018fairness,biega2018equity,morik2020controlling}): $\forall k \in \intint{K}, \ew_k = \frac{1}{\log_2(1+k)}.$ %and $\forall k \in \{K+1, \ldots,m\}, \ew_k = 0.$

The generated $\muij$ are used as ground truth to evaluate rankings, in order to decouple the fairness evaluation of the ranking algorithms from the evaluation of biases in preference estimates (which are not addressed in the paper). The results are the average of three repetitions of the experiments over different random train/valid/test splits used to generate the $\mu_{ij}$.


\subsubsection{Defining the GGF weights $\protect\bw$} 

We study 3 different weighting functions for GGF, which are used for users ($\ubw$) and/or items ($\ibw$). 
\begin{enumerate}
    \item \Gini: weights of the classical Gini index: $w_i = \frac{n - i + 1}{n}$
    \item \Bonfer: weights of the Bonferroni index \citep{bonferroni1941elementi,aristondo2013}: $w_i = \sum_{\ell=i}^n \frac{1}{\ell n}$
    % \item \geom weights: $\bw_i = \frac{1}{2^{i-1}}$ as in \cite{busa2017multi}
    % \item \quantile trade-off between total utility and cumulative utility of the $\floor{\nicefrac{i}{n}}$\%-worse-off individuals. \quantile is specified by two parameters $(i, \omega) \in \intint{n} \times [0,1]$, where $\lw_{i} = \omega\,$,  $\lw_n = 1 - \omega,$ and $\lw_j = 0$ for $j\neq i, n$. The $\lw$ are then converted from the Lorenz space to $\bw$ in the space of GGF weights.
    \item \quantile trade-off between total utility and cumulative utility of the $q$\%-worse-off users or items. \quantile is specified by two parameters $(q, \omega) \in [0,1]^2$, where $\lw_{i} = \omega\,$,  $\lw_{\floor{qn}} = 1 - \omega,$ and $\lw_j = 0$ for $j\neq \floor{qn}, n$. The $\lw$ are then converted from Lorenz space to $\bw$ in the space of OWA weights. This approach is reminiscent of quantile ratios in the literature on inequality measures.
\end{enumerate}

\subsubsection{Fairness objectives}

In our experiments, we compare our two-sided GGF objective \eqref{eq:owaobj} to  existing approaches to fairness in rankings, where a parameter $\iw$ controls the trade-off between a user objective and an item objective.

\nico{I think here it is not super clear what the task is or why these baselines are relevant}

\paragraph{FairRec \citep{patro2020fairrec}}\citet{patro2020fairrec} study two-sided fairness in recommendation.\footnote{\citep{patro2020fairrec} consider unordered recommendation lists with a uniform attention model. We transform them into ordered lists using the order output by \patro, and adapt the item-side criterion of minimal exposure to the position-based model.} Their algorithm \patro guarantees envy-freeness for users, and a minimum exposure of $\frac{\lambda n\norm{\ew}}{m}$ for every item. %$\lambda$ is the parameter of \patro which controls the trade-off between their notions of user-side and item-side fairness.

The following two objectives are smooth concave objective functions that we maximize using the tractable Frank-Wolfe method for ranking from \citep{do2021two}.

\paragraph{Social welfare (\welf)} \citet{do2021two} address two-sided fairness in rankings by maximizing concave welfare functions of user utilities and item exposures:
\begin{align}\label{eq:def-qua}
    &F^\welf(P) = (1-\lambda) \sum_{i=1}^n \phi(u_i(P), \alpha_1) +  \lambda \sum_{j=1}^m \phi(v_j(P), \alpha_2)\\
    &\text{where }~ \phi(x, \alpha)=\begin{cases}
    x^\alpha&\text{~if~} \alpha>0\\
    \log(x)&\text{~if~}\alpha=0\\
    -x^\alpha&\text{~if~}\alpha<0
    \end{cases}.
\end{align}
 Lower values of $\alpha_1$ (resp. $\alpha_2$) drive towards more redistribution of utility in the user (resp. item) population, while $\lambda$ controls the tradeoff between the social welfare of users and items.

\paragraph{Equal exposure (\equalexpo)} Several authors \cite{singh2018fairness,wu2021tfrom} advocate for item-side fairness in the sense of equal exposure across (groups) of items. In the following objective \citep{do2021two}, this fairness requirement takes the form of a smooth and concave penalty which is traded against the overall utility of users:
\begin{align}\label{eq:def-eq-expo}
    F^\util(P) = \sum_{i=1}^n u_i(P) -  \frac{\lambda}{m}\sqrt{\sum_{j=1}^m\left(v_j(P) - \frac{1}{m} \sum_{j'=1}^m v_{j'}(P)\right)^2}
\end{align}

Due to space constraints, we do not include a comparison with the related criterion of \emph{``equity of exposure''} \citep{biega2018equity,diaz2020evaluating}, also called  \emph{``merit-based fairness''} \cite{singh2019policy}, because it is formally similar to \equalexpo, by replacing $v_j(P)$ with $\nicefrac{v_j(P)}{q_j}$ where $q_j = \sum_{i=1}^n \muij$ is a measure of the ``merit'' of $j.$ For a comparison with GGF, we would simply need to replace $\iGGF(\bv(P))$ with $\iGGF(\bv(P) / \xvector{q})$.

% \paragraph{Quality-weighted exposure (\qualexpo)} A major item-side fairness criterion\footnote{It has been called \emph{``merit-based fairness''} \cite{singh2019policy}, \emph{equity of exposure} \citep{biega2018equity,diaz2020evaluating} and \emph{``quality-weighted exposure''} \citep{wu2021tfrom,do2021two}.} requires that the total exposure of an item should be proportional to a measure of its quality \cite{singh2018fairness,biega2018equity,diaz2020evaluating,wu2021tfrom}:
% \begin{align}\label{eq:def-qua}
%     &F^\gqua(P) = \sum_{i=1}^n u_i(P) -  \frac{\lambda}{m}\sqrt{\sum_{j=1}^m\left(v_j(P) - \frac{1}{m} \sum_{j'=1}^m q_{j'}\frac{ n\norm{\ew}_1}{Q}\right)^2}\\
%     &\text{where }~ q_j = \sum_{i=1}^n \muij ~~\text{ and } ~~ Q = \sum_{j'=1}^m q_{j'}. \end{align}


\paragraph{Sum user utility and GGF for items} We also consider the special case where $F(P)$ is a trade-off function between the total user utility and item fairness specified by a GGF, by setting $\ubw = (1, \ldots, 1)$:
\begin{align}\label{eq:item-GGF}
    F(P) =  (1- \iw) \sum_{i=1}^n u_i(P) + \iw g_{\ibw}(\bv(P)).
\end{align}
When %$\ibw_j=\frac{2 ( m- j) + 1}{m^2}$
$\ibw = \Gini$, maximizing the second term in $F(P)$ is equivalent to minimizing inequalities between items measured by the Gini index. This approach is similar to \equalexpo, except that the latter minimizes item inequalities measured by the standard deviation (std).


\subsection{Convergence diagnostics} \label{sec:xp-convergence}

\begin{figure}
\centering 
\subfigure[\lastfmsmall ($\iw=0.5, \mathbf{w^2}=\Gini)$]{\label{fig:lastfm-gini-cvg}\includegraphics[width=0.49\linewidth]{figures/convergence/cvg_classicgini_lastfmsmall.png}}
\subfigure[MovieLens ($\iw=0.5, \mathbf{w^2}=\Gini)$]{\label{fig:ml20m-gini-cvg}\includegraphics[width=0.49\linewidth]{figures/convergence/cvg_classicgini_ml20m.png}}
% \subfigure[\lastfmsmall ($\iw=0.99, w^2_i=\frac{1}{2^{i-1}}$) ]{\label{fig:lastfm-geom-cvg}\includegraphics[width=0.49\linewidth]{figures/convergence/cvg_geometric_lastfmsmall.png}}
% \subfigure[MovieLens ($\iw=0.99,  w^2_i=\frac{1}{2^{i-1}}$)]{\label{fig:ml20m-geom-cvg}\includegraphics[width=0.49\linewidth]{figures/convergence/cvg_geometric_ml20m.png}}
\subfigure[\lastfmsmall ($\iw=0.99, \protect\ibw=\Bonfer$) ]{\label{fig:lastfm-bonfer-cvg}\includegraphics[width=0.49\linewidth]{figures/convergence/cvg_bonferroni_lastfmsmall.png}}
\subfigure[MovieLens ($\iw=0.99,  \protect\ibw=\Bonfer$)]{\label{fig:ml20m-bonfer-cvg}\includegraphics[width=0.49\linewidth]{figures/convergence/cvg_bonferroni_ml20m.png}}

\caption{\label{fig:convergence-smoothing-subgradient}Convergence of \fwsubgrad compared to \fwsmooth, for various values of $\beta_0.$ \fwsubgrad fails to converge to the optimal GGF value.}
\end{figure}


We first demonstrate the usefulness of \fwsmooth for optimizing  GGF objectives, compared to simply using the Frank-Wolfe method of \citep{do2021two} with a subgradient (\fwsubgrad) of the GGF given in Sec. \ref{sec:algo-challenge}. More precisely, \fwsubgrad is also equivalent to using a subgradient of $f = -F$ in $\rrkt$ in Line 3 of Alg. \ref{alg:nonsmoothfw}, instead of $\grad \fbetat (\rrkt), $ thus ignoring the smoothing parameters $\beta_t$. 


% Then the baseline we consider is the Frank-Wolfe method of \citep{do2021two}, where the direction step $~~\Qt = \argmin\limits_{\rrk\in\rrkS} \xdp{\rrk}{\grad F(P^{(t)}})~~$ takes a subgradient of $F$ instead, and is obtained with the top-$K$ ranking that sorts $\tmuij \gets \ubw_{\pi_1^{-1}(i)} \muij + \ibw_{\pi_2^{-1}(j)} \mu_{ji}$ for each user $i, $ where  $\pi_1 \gets \argsort\sort(\bu(\rrkt))$ and $\pi_2\gets \argsort\sort(\bv(\rrkt)).$

%%%%


\fwsubgrad is simpler than our \fwsmooth method, and its complexity is of the same order, but \fwsubgrad runs faster in practice because it does not involve the sorting and isotonic regression required to compute the gradient of the smoothed objective $\fbetat$. However, it was previously shown that replacing gradients with subgradients in Frank-Wolfe does not guarantee convergence \citep{nesterov2018complexity}. 

We show that this prevents us from using \fwsubgrad in practice despite its appealing properties. We optimize $F(P)$ with form \eqref{eq:item-GGF} and item weights $\ibw \in \{\Gini,\Bonfer\}$ on \lastfmsmall and MovieLens, using \fwsubgrad and \fwsmooth with different values of $\beta_0$. Figure 
\ref{fig:convergence-smoothing-subgradient} depicts the objective value as a function of the number of iterations, averaged over three seeds (the colored bands represent the std). On \lastfmsmall, we observe that for both \Gini and \Bonfer (Fig \ref{fig:lastfm-gini-cvg} and \ref{fig:lastfm-bonfer-cvg}), \fwsubgrad (blue dotted curve) plateaus at a suboptimum. In contrast, \fwsmooth converges (orange and green curves), and the convergence is faster for larger $\beta_0$. On MovieLens, \fwsubgrad converges for the \Gini objective (Fig \ref{fig:ml20m-gini-cvg}), but not the \Bonfer one (Fig. \ref{fig:ml20m-bonfer-cvg}). 

Hence \fwsubgrad is not a reliable option for optimizing GGFs, while the algorithm we propose has strong convergence guarantees and comparable computational complexity.



\subsection{Multiplicity of fairness trade-offs} \label{sec:xp-onesided-tradeoff}



\begin{figure}
\centering    
\subfigure[Total user utility (higher is better)]{\label{fig:lastfm-total}\includegraphics[width=0.49\linewidth]{figures/pareto_fronts/lastfmsmall/Giniitem-user_utility-lastfmsmall-42.png}}
\subfigure[Inequalities among users (lower is better)]{\label{fig:lastfm-ineq}\includegraphics[width=0.49\linewidth]{figures/pareto_fronts/lastfmsmall/Giniitem-Giniuser-1sided-alpha1-lastfmsmall-42.png}}
\subfigure[Utility of the 25\% worse-off users (higher is better)]{\label{fig:lastfm-user25}\includegraphics[width=0.49\linewidth]{figures/pareto_fronts/lastfmsmall/Giniitem-first25u-1sided-alpha1-lastfmsmall-42.png}}
\subfigure[Utility of the 50\% worse-off users (higher is better)]{\label{fig:lastfm-user50}\includegraphics[width=0.49\linewidth]{figures/pareto_fronts/lastfmsmall/Giniitem-first50u-1sided-alpha1-lastfmsmall-42.png}}
\caption{\label{fig:lastfm-userfairness}Trade-offs between various user fairness objectives and item-side inequalities on \lastfmsmall. The Pareto fronts are generated by varying $\iw$. For (c) and (d), the user-side GGF weights $\protect\ubw$ are generated via \quantile, with $(q,\omega) \in \{0.25,0.5\} \times \{0.25,0.5,0.1\}.$ }
\end{figure}

\begin{figure}
\centering    
\subfigure[Total user utility (higher is better)]{\label{fig:ml20m-total}\includegraphics[width=0.49\linewidth]{figures/pareto_fronts/ml20m/Giniitem-user_utility-ml20m-42.png}}
\subfigure[Inequalities among users (lower is better)]{\label{fig:ml20m-ineq}\includegraphics[width=0.49\linewidth]{figures/pareto_fronts/ml20m/Giniitem-Giniuser-1sided-alpha1-ml20m-42.png}}
\subfigure[Utility of the 25\% worse-off users (higher is better)]{\label{fig:ml20m-user25}\includegraphics[width=0.49\linewidth]{figures/pareto_fronts/ml20m/Giniitem-first25u-1sided-alpha1-ml20m-42.png}}
\subfigure[Utility of the 50\% worse-off users (higher is better)]{\label{fig:ml20m-user50}\includegraphics[width=0.49\linewidth]{figures/pareto_fronts/ml20m/Giniitem-first50u-1sided-alpha1-ml20m-42.png}}
\caption{\label{fig:ml20m-userfairness} Trade-offs between various user fairness objectives and item-side inequalities on MovieLens. }
\end{figure}

\virginie{TODO: I should no longer talk about Lorenz efficiency here}

We now present experiments that illustrate the result of Prop. \ref{lem:all-lorenz}: since GGF allows to generate every Lorenz efficient ranking, it allows reach the best possible tradeoff between \emph{any} criteria compatible with Lorenz efficiency.


For each fairness objective, Pareto frontiers are generated by varying $\iw$. We compare ourselves to \welf with the parameters $\alpha_2=0$ recommended in \citep{do2021two} (and $\alpha_1 =\in \{-2,0,1\}$). Since \citet{patro2020fairrec}'s algorithm \patro does not scale, we compare to \patro only on \lastfmsmall. 

We optimize $F(P)$ using \fwsmooth with $\beta_0=100$ and $T=5k$ for \lastfmsmall, and $\beta_0=1000$ and $T=50k$ for MovieLens. $F^\welf$ and $F^\util$ are optimized with the Frank-Wolfe method of \citep{do2021two} for $T=1k$ and $T=5k$ iterations respectively for \lastfmsmall and MovieLens. This is the number of iterations recommended by \citep{do2021two}, while we need more interactions for \fwsmooth because its convergence is $O(\frac{1}{\sqrt{T}})$ rather than $O(\frac{1}{T})$ because of non-smoothness.

We first analyze the fairness tradeoffs achieved on \lastfmsmall (Figure \ref{fig:lastfm-userfairness}). \emph{Fig. \ref{fig:lastfm-total}}: On the usual trade-off between total utility of users and Gini inequalities between items, GGF (``red +'' curve) obtains the best trade-off. This is done by using the form \eqref{eq:item-GGF} with the classical \Gini weights for items. It fares better than \equalexpo (orange $\times$) on this specific trade-off because \equalexpo reduces inequalities between items by minimizing the std of exposures, while GGF with \Gini weights minimizes the Gini index. 


\emph{Fig. \ref{fig:lastfm-ineq}}: Our two-sided GGF objective \eqref{eq:owaobj} also accounts for user fairness. Looking at tradeoffs between user inequalities and item inequalities, we observe that GGF with \Gini weights for both users and items (red curve) leads to the lowest inequalities between users, at all levels of inequalities between items. It indeed outperforms \equalexpo (orange) which does not consider user fairness, and \patro's user criterion (blue) that does not aim to reduce inequalities.


GGF is general enough to address a larger variety of fairness criteria than those based on inequalities. \emph{Fig. \ref{fig:lastfm-user25} and \ref{fig:lastfm-user50}} showcase the tradeoffs achieved by various methods between the utility of the $25\%$ / $50\%$ worst-off users and inequalities among items. These Pareto fronts illustrate the fairness requirement that worse-off fractions of the user population should not bear the cost of reducing inequalities between items. We set $\alpha_2=-2$ in \welf (orange) because it was previously reported to achieve a good performance on these criteria in \citep{do2021two}. As expected, it is outperformed by our two-sided GGF approach (purple) with \quantile weights on the $25 \%$ (resp. $50 \%)$ worse-off users, and \Gini weights on the item-side. As expected, the more weight is put on the $25 \%$ worst-off in GGF, the higher the curve, which is why we observe the ordering green < red < purple for GGF. The combination of paramaters $\ubw,\ibw=(\quantile,\Gini)$ is exactly designed to optimize the tradeoffs illustrated in Fig. \ref{fig:lastfm-user25} and \ref{fig:lastfm-user50}.

Figure \ref{fig:ml20m-userfairness} shows the same panel of tradeoffs on MovieLens. Results are qualitatively similar: by adequately parameterizing GGF, it reaches the best tradeoff on all criteria. %This shows that the \fwsmooth algorithm is able to scale to larger datasets and converge to optimal fairness tradeoffs.


Overall, there are a plethora of criteria to assess the fairness of ranking methods, and the choice of criteria is application-dependent. These experiments show that our two-sided GGF approach provides enough control to satisfy a large panel of fairness desiderata, by reaching the best possible fairness trade-off among \emph{all} Lorenz efficient rankings (as shown theoretically in Section \ref{sec:gini}). 



% \subsection{Fairness trade-offs in reciprocal recommendation} \label{sec:xp-reciprocal}


% \begin{figure}
% \centering    
% \subfigure[Total utility vs. inequalities (higher is better)]{\label{fig:twitter13k-total}\includegraphics[width=0.49\linewidth]{figures/pareto_fronts/twitter13k/Giniuser-user_utility-twitter13k-42.png}}
% \subfigure[Total utility vs. utility of the 10\% worse-off (higher is better)]{\label{fig:twitter13k-user10}\includegraphics[width=0.49\linewidth]{figures/pareto_fronts/twitter13k/Giniuser-user_utility-first10-twitter13k-42.png}}
% \subfigure[Total utility vs. utility of the 25\% worse-off (higher is better)]{\label{fig:twitter13k-user25}\includegraphics[width=0.49\linewidth]{figures/pareto_fronts/twitter13k/Giniuser-user_utility-first25-twitter13k-42.png}}
% \subfigure[Total utility vs. utility of the 50\% worse-off (higher is better)]{\label{fig:twitter13k-user50}\includegraphics[width=0.49\linewidth]{figures/pareto_fronts/twitter13k/Giniuser-user_utility-first50-twitter13k-42.png}}
% \caption{Fairness trade-offs on Twitter. The Pareto fronts are generated by varying $\lambda$ in \equalu, and $\alpha$ in \welf. The GGF weights $\protect\bw$ are generated via \quantile, with $q \in \{0.1, 0.25,0.5\}$ and we vary $\omega$ to generate the curves. [TODO: replace one of the squares with Lorenz curves?\label{fig:twitter13k-paretofronts}] [fig. a is todo ]}
% \end{figure}

% \paragraph{Data} We simulate a friend recommendation task from the Higgs \textbf{Twitter} dataset \citep{de2013anatomy}, which contains directed follower links on the social network Twitter. We consider a mutual follow as a ``match'', and we keep users having at least 20 matches, resulting in a subset of $13k$ users. We estimate mutual scores $\muij$ (i.e., match probabilities) by matrix factorization.

% \paragraph{Fairness objectives} We compare GGF to the \emph{equal utility} objective (\equalu) which penalizes inequalities in utilities between users in reciprocal recommendation \citep{do2021two}, as measured by the std:

% \begin{align}\label{eq:def-eq-util}
%     F^\util(P) = \sum_{i=1}^n u_i(P) -  \frac{\lambda}{n}\sqrt{\sum_{i=1}^n\left(u_i(P) - \frac{1}{n} \sum_{i'=1}^n u_{i'}(P)\right)^2}.
% \end{align}

% We also compare to \welf for reciprocal recommendation \citep{do2021two}, where a single parameter $\alpha$ controls the redistribution among users.


% \paragraph{Fairness trade-offs results} We now demonstrate that in reciprocal recommendation too, GGF obtains the best trade-offs between multiple fairness criteria. We optimize $F$ using \fwsmooth with $\beta_0=10$ for $T=150k$ iterations, and optimize $F^\welf$ and $F^\util$ using Frank-Wolfe for $T=5k$ iterations.

% Figure \ref{fig:twitter13k-paretofronts} depicts the trade-offs between total utility and various fairness criteria achieved by the competing approaches. On Fig. \ref{fig:twitter13k-total}, GGF (xxx curve, TODO) uses the weights:
% $\bw = \lambda + (1 - \lambda) * \Gini$ and varying $\lambda.$ This form of GGF is designed for the optimization of tradeoffs of the form \emph{``total utility vs. inequalities measured by Gini index''}, which is why GGF dominates competing approaches on Fig. \ref{fig:twitter13k-total}. As in one-sided recommendation, the reason why \equalu achieves worse trade-offs on this comparison is because it minimizes the std instead of the Gini index.


% On Fig. \ref{fig:twitter13k-user10},\ref{fig:twitter13k-user25},\ref{fig:twitter13k-user50}, we observe that for trade-offs of the form \emph{``total utility vs. utility of the $q$\% worse-off''}, GGF with $q$ \quantile weights (green curve) is the most effective. 




==> sections/old/fairranking.tex <==
\section{Two-sided Fairness in rankings with Generalized Gini Welfare functions} \label{sec:ggf-ranking} 

In this section, we show how the GGFs introduced in Section \ref{sec:gini} and the smoothing approach described in Section \ref{sec:moreau-ggf} can be leveraged to generate rankings that are fair towards users and items in a recommender system.

\subsection{Recommendation framework}\label{sec:framework}

We consider a recommendation scenario with $n$ users, and $m$ items, and $K$ recommendation slots. $\mu_{ij} \in [0,1]$ denotes the value of item $j$ for user $i$ (e.g, a ``liking'' probability), and we assume the values $\mu$ are given as input to the recommender system. 

The goal of the system is to produce a ranked list of items for each of the $n$ users. %Formally, for all $i \in \intint{n},$ the recommender system outputs $\sigma_i, $ a permutation of $\intint{m}$, such that $\sigma_i(j)$ is the rank of item $j$ in the list shown to user $i.$ 
Following previous work on fair rankings \citep[e.g.][]{singh2018fairness}, we consider stochastic rankings because they enable (a) the use of convex optimization techniques, and (b) redistribution of exposure, in contrast to deterministic rankings where the same items capture most attention \nico{I'm not sure the end of the sentence is clear} \virginie{I meant to say it gives us ``du mou pour la redistribution''}. A stochastic ranking for user $i$ is represented by a bistochastic matrix $\rrk_i \in \reals^{m\times m},$ where $\rrk_{ijk}$ is the probability that item $j$ is recommended to user $i$ at position $k.$ The recommender system outputs a \emph{stochastic ranking policy} $\rrk = (\rrk_i)_{i=1}^n$, and we denote the convex set of stochastic ranking policies by $\rrkS$.

In line with previous work, we consider a position-based model with non-increasing weights $\ew \in \reals_+^m,$ where $\ew_k$ is the probability that a user examines the item at position $k.$ Since there are $K$ recommendation slots, we have $\ew_1 \geq \ldots \geq \ew_K$ and $\ew_k = 0$ for any $k > K.$ 

Since the recommender system impacts both user and items, we model this two-sided impact through two notions of utility. The user utility is defined as the expected performance of the ranking for the user in the position-based model, and the item utility is their average total exposure to users:
\begin{align*}
    \textit{User utility: }\, u_i(P) = \sum_{j=1}^m \muij \rrk_{ij} \ew &&\textit{Item exposure: }\, v_j(P) = \sum_{i=1}^n\rrk_{ij} \ew
\end{align*}

The generalized Lorenz curves of users and items are respectively denoted $\bucum(P)$ and $\xvector{V}(P)$.

Fairness in recommender systems is often studied at the level of social groups. Our framework extends to this setting by defining the utility (resp. exposure) of a group of users (resp. item) by taking the sum or average of utilities of its members, as in prior work \citep{singh2018fairness,morik2020controlling}. We present our framework for individuals to (a) keep the presentation simple, and (b) to show that considering fairness towards each individual is not a bottleneck -- in particular, since our method is tractable for individuals, it is also tractable for multiple intersectional subgroups \citep{kearns2017preventing,hebert2017calibration}.
%The set of feasible utility profiles is $\US= \{(\bx, \by) \in \reals^n \times \reals^m \,:\, \exists \rrk \in \rrkS, \bx = \bu(\rrk) ~ \text{and} ~ \by = \bv(\rrk) \}.$ 


\subsection{Objective: two GGFs for two-sided fairness} \label{sec:2sided-ggf-obj}

In the recommendation setting, the multiobjective problem consists in optimizing each point of the generalized Lorenz curves of both users and items, over the set of stochastic ranking policies $\rrkS$: $\,
    \max\limits_{\rrk \in \rrkS}\, (U_1(P),\ldots, U_n(P), V_1(P),\ldots V_m(P)).$
    
For $(\iw, \ulw, \ilw) \in [0,1]\times \reals_+^n \times \reals_+^m$ s.t. $\,\sum_{i=1}^n \ulw_i = 1$ and $\sum_{j=1}^n \ilw_j = 1$, the weighted sum objective is: 
\begin{align}\label{eq:mainobj}
    \max_{\rrk \in \rrkS} \, \,\left\{ F(P) :=(1-\iw) \sum_{i=1}^{n}\ulw_i U_i(P) + \iw \sum_{j=1}^{m} \ilw_j V_j(P) \right \}.
\end{align}

The choice of $\ilw_j$ controls the degree of priority to the $\frac{j}{m}$-$\%$ worse-off items, and $\ulw_i$ is for the $\frac{i}{n}$-$\%$ worse-off users, while $\iw$ controls the relative weight of users and items. Overall, there are two coarse-grained objectives, one for users and one for items, and many fine-grained objectives for each individual of either populations.

Denoting $\ubw_i = \sum_{l=i}^n \ulw_l\,$ and $\ibw_j = \sum_{l=j}^m \ilw_l\,$, the main objective is then a weighted sum of two GGFs, one for users and one for items: %ordered weighted averages (OWAs) of utilities with nonincreasing positive weights $\ubw$ and $\ilw$: _1 \geq \ldots \geq \ubw_n > 0 $, and $\ibw_1 \geq \ldots \geq \ibw_m > 0 $:
\begin{align}\label{eq:owaobj}
    &F(P) = (1- \iw) g_{\ubw}(\bu(P)) + \iw g_{\ibw}(\bv(P)).
\end{align} 
% \begin{align}\label{eq:owaobj}
%     &F(P) = G(\bu(P), \bv(P)) \\
%     &\text {with }~G(\bx, \by) = (1- \iw) g_{\ubw}(\bx) + \iw g_{\ibw}(\by).
% \end{align} 
% \begin{align}
%     F(P) := \iw \sum_{i=1}^{n}\ubw_i u_i\sort(P) + (1-\iw) \sum_{j=1}^{m}\ibw_j v_j\sort(P).
% \end{align}

% Our goal is to maximize $F(P)$ which balances between a GGF for users and a GGF for items. The fact that the OWA weights are decreasing gives priority to the worse-off, and favors transfers from better-off to worse-off. The parameters of $F(P)$ allow to control the complex multi-dimensional trade-off between users and items' utilities. 

\virginie{At this stage is it clear that it leads to fair solutions? I expect the Section on Gini to set the stage. I can also briefly mention Lo-efficiency here (no formal definition)}


\subsection{Frank-Wolfe with smoothing} \label{sec:fwsmooth}

\virginie{Insert a few words on the LP approach here?}

We consider the minimization of $f := -F$ over $\rrkS,$ and for any $\beta > 0$, we define the smooth approximation of $f$ as $\fbeta(P) := (1-\iw) h_1^\beta(\bu(P)) + \iw h_2^\beta(\bv(P)),$ which is a linear combination of the Moreau envelopes of $-\uGGF$ and $-\iGGF.$

Our algorithm (\fwsmooth) for minimizing $f$ is the Frank-Wolfe method for nonsmooth optimization from \citep{lan2013complexity} which constructs iterates $P^{(t)}$ at each iteration $t \leq T$ and outputs a stochastic ranking policy $\rrk^{(T)}.$ Given a positive sequence $(\beta_t)_{t\geq 1}$ decreasing to $0$, at each iteration $t$, the algorithm takes a direction search step with respect
to the smooth approximation $\fbetat$ of $f$, by calculating:
\begin{align}\label{eq:fw-step}
    &\Qt = \argmin_{\rrk\in\rrkS} \xdp{\rrk}{\grad \fbetat(P^{(t))}}.
\end{align}
$\rrk^{(0)}$ is initialized as a deterministic ranking policy, e.g. such that $\rrk^{(0)}_i$ represents a permutation in $\topk (\mui)$. $\rrkt$ is updated as:
\begin{align}\label{eq:fw-update}
    \rrk^{(t+1)} \gets \left(1 - \frac{2}{t + 1}\right)  \rrkt + \frac{2}{t + 1} \Qt.
\end{align}
\virginie{Would it be better if I present Lan's algorithm in an Algoritm environment?}\nico{and maybe in the previous section?}


\begin{algorithm}
    \caption{\label{alg:fwsmooth-step}Direction search in \fwsmooth \eqref{eq:fw-step}}
    \DontPrintSemicolon
     \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
     
     \Input{utilities $\bu(\rrkt)$, smoothing $\sm_t$, weights $\ibw,\ubw$}
     \Output{deterministic ranking policy $\Qt$}
     $\ubw \gets -(\ubw_n,...,\ubw_1)~$ and $~\ibw \gets -(\ibw_n,...,\ibw_1)$\;
     $\pi_1 \gets \argsort\descsort(\frac{\bu(\rrkt)}{\beta_t})~$ and $~\pi_2 \gets \argsort\descsort(\frac{\bv(\rrkt)}{\beta_t})$\;
     $\bz^1 \gets \frac{\bu(\rrkt)}{\beta_t}~$ and $~\bz^2 \gets \frac{\bv(\rrkt)}{\beta_t}$\;
     $\bx^1 \gets \PAV(\bz^1_{\pi_1} - \ubw)~$ and $~\bx^2 \gets \PAV(\bz^2_{\pi_2} - \ibw)$\;
     $\uyt \gets \bz^1 + \xvector{x^1_{\pi_1^{-1}}}~$ and $~\iyt \gets \bz^1 + \xvector{x^2_{\pi_2^{-1}}}$\;
     \For{i=1, \ldots, \n}{
          $\tempmuij \gets (1-\iw) \uyt_i \muij + \iw \iyt_j$ \;
          $~~\tilde{\sigma}_i \gets \topk( -\tilde{\mu}_i )$} Return $\Qt \in \rrkS$ such that $\Qt_i$ represents  $\tilde{\sigma}_i$.\;
\end{algorithm}


\paragraph{Efficient computation of the Frank-Wolfe direction step} Frank-Wolfe methods are advantageous when step \eqref{eq:fw-step} can be computed efficiently, which was shown to be the case for smooth ranking objectives \citep{do2021two}. Similarly, in our case, the form of $\grad \fbeta(P)$ given by Lemma \ref{lem:moreau} as a function of $\bu^*$ enables to solve step \eqref{eq:fw-step}  with only one top-$K$ sorting operation per user. 


% \begin{proposition}[Th. 1, \citet{do2021two}]\label{prop:fwgrad}
% Let $\yt = \frac{1}{\beta_t}(\bu(P^{(t)})- \prox_{\beta_t h}(\bu(P^{(t)}))$ and $\tempmuij = \yt_i \muij$. For all $i \in \intint{n},$ let $\tilde{\sigma}_i \in \topk(\tilde{\mu}_i)$ and $\Qt_i$ a permutation matrix representing $\tilde{\sigma}_i$.
% Then $\Qt \in \argmin\limits_{\rrk \in \rrkS} \xdp{\rrk}{\grad \fbetat(\rrkt)}.$
% \end{proposition}

\begin{proposition}\label{prop:fwgrad}
Let $\uyt=\proj_{\ph({\utbw})}\left(\frac{\bu(\rrkt)}{\sm_t}\right)$ and $\iyt=\proj_{\ph({\itbw})}\left(\frac{\bv(\rrkt)}{\sm_t}\right).$ Let $\tempmuij = (1-\iw) \uyt_i \muij + \iw \iyt_j$. For all $i \in \intint{n},$ let $\tilde{\sigma}_i \in \topk(-\tilde{\mu}_i)$ and $\Qt_i$ a permutation matrix representing $\tilde{\sigma}_i$.
Then $\Qt \in \argmin\limits_{\rrk \in \rrkS} \xdp{\rrk}{\grad \fbetat(\rrkt)}.$
\end{proposition}

\begin{proof}
Using the expression of the gradient of the Moreau envelope derived in Section \ref{sec:isotonic}, eq. \eqref{eq:yt-proj}, we have:\begin{align*}
    \grad \fbeta(P) = (1 - \iw) \, \bu^* (\proj_{\ph(\utbw)}\left(\nicefrac{\bu(P)}{\beta}\right)) + \iw \, \bv^* (\proj_{\ph(\itbw)}\left(\nicefrac{\bv(P)}{\beta}\right))
\end{align*}

By definition of $\uyt,\iyt$, for all $\rrk \in \rrkS$ we have: \begin{align*}
    \xdp{\rrk}{\grad \fbetat(P^{(t)}}) &= (1 - \iw) \xdp{\rrk}{\bu^* (\uyt)} + \iw \xdp{\rrk}{\bv^* (\iyt)}) \\
    &= (1 - \iw) \xdp{\bu(P)}{\uyt} + \iw \xdp{\bv(P)}{\iyt}\\
    &= (1 - \iw) \sum_{i=1}^n\sum_{j=1}^m  \uyt_i \muij  \rrk_{ij} \ew + \iw \sum_{j=1}^m \sum_{i=1}^n \iyt_j \rrk_{ij} \ew \\
    %&= \sum_{i=1}^n\sum_{j=1}^m  \left((1 - \iw) \uyt_i \mu_i^\intercal + \iw \iyt_j  \right) \rrk_{ij} \ew.
    &= \sum_{i=1}^n\sum_{j=1}^m  \tempmuij \rrk_{ij} \ew.
\end{align*}
The result follows from Lem. 3 of \citep{do2021two} and is a consequence of the rearrangement lemma \cite{hardy1952inequalities}: the optimal $\Qt \in \argmin\limits_{\rrk \in \rrkS} \xdp{\rrk}{\grad \fbetat(\rrkt)}$ is obtained by sorting $\tempmuij$ in increasing order (or equivalently, $-\tempmuij$ in decreasing order since we consider the minimization of $f=-F$).
\end{proof}


% \paragraph{Summary of step \eqref{eq:fw-step}} Using \eqref{eq:prox}, the vector $\yt$ of Proposition \ref{prop:fwgrad} simply writes as the projection
% \begin{equation}
% \begin{aligned}
%     \yt =  \proj_{\ph(\tbw)}\left(\frac{\bu(\rrkt)}{\sm_t}\right),
% \end{aligned}
% \end{equation}
% and is computed by the formula of Proposition \ref{prop:isoto} using the Pool Adjacent Violators algorithm. The solution of step \eqref{eq:fw-step} is then obtained as a $\topk(\yt_i\mu_i)$ for each user $i$. Our full algorithm is described in Alg. \ref{alg:full}, App. \ref{app:morealgo}.


\paragraph{Algorithm and theoretical guarantees} Algorithm \ref{alg:fwsmooth-step} describes the computation of the Frank-Wolfe direction step \eqref{eq:fw-step}, summarizing the results of Section \ref{sec:isotonic} and Prop. \ref{prop:fwgrad}. The full 
\fwsmooth algorithm consists in running Alg. \ref{alg:fwsmooth-step} for $T$ iterations with $\beta_t > 0$ decreasing to 0, as in the template of \citet[Sec. 3.2][]{lan2013complexity}. The convergence guarantee is:

\begin{proposition}[Th. 4, \citet{lan2013complexity}]\label{prop:converge} With $\beta_0 = \frac{2 D_{\rrkS} \|\bu\|}{\|\bw\|} $ and $\beta_t = \frac{2}{\sqrt{t+1}}$, \fwsmooth obtains the following convergence rate: $$f(P^{(T)}) - f(P^*) \leq \frac{2 D_{\rrkS} \|\bu\|\|\bw\|}{\sqrt{T+1}}.$$
\end{proposition}


Combining Propositions \ref{prop:isoto} and \ref{prop:fwgrad}, we obtain the following complexity result:

\begin{proposition}\label{prop:complexity} Algorithm \ref{alg:fwsmooth-step} runs with $O(n \ln n + m \ln m)$ operations per user and requires $O(n + m)$ memory.
\end{proposition}

When running the full \fwsmooth algorithm for $T$ iterations, the storage requirement is $O((n + m) \times T).$ 
 Moreover, the algorithm provides a \emph{sparse representation of the stochastic rankings} as a weighted sum of permutation matrices, since $\rrkt$ is updated using the linear combination of eq. \eqref{eq:fw-update}. In other words, this gives us a Birkhoff-von-Neumann decomposition \cite{birkhoff1940lattice} of the bistochastic matrices \emph{for free}, avoiding the overhead of an additional decomposition algorithm as in existing works on fair ranking \citep{singh2018fairness,wang2020fairness,su2021optimizing}. 






% \begin{algorithm}\label{alg:fwsmooth-step}
%     \caption{Frank-Wolfe direction step \eqref{eq:fw-step}}
%     \DontPrintSemicolon
%      \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
     
%      \Input{utilities $\bu(\rrkt)$, smoothing $\sm_t$, weights $\bw$}
%      \Output{deterministic ranking $\Qt$}
%      $\sigma \gets \argsort\descsort(\frac{\bu(P^{(t)})}{\beta_t})$ and  $\bz \gets \frac{\bu(P^{(t)})}{\beta_t}$\;
%      $\bx \gets \PAV(\bzsig - \bw)$\;
%      $\yt \gets \bz + \xvector{x_{\sigma^{-1}}}$\;
%      \lFor{i=1, \ldots, \n}{
%          $\tilde{\mu}_i \gets \yt_i \mui~$ and $~~\tilde{\sigma}_i \gets \topk( \tilde{\mu}_i )$} Return $\Qt \in \rrkS$ such that $\Qt_i$ represents  $\tilde{\sigma}_i$.\;
% \end{algorithm}



==> sections/old/framework.tex <==
\section{Fair ranking with Generalized Gini} \label{sec:framework} 
% that's the worst section title ever, but let's bear with that for now

\subsection{Recommendation framework}%\label{sec:framework}

We consider a recommendation scenario with $n$ users, and $m$ items, and $K$ recommendation slots. $\mu_{ij} \in [0,1]$ denotes the value of item $j$ for user $i$ (e.g, a ``liking'' probability), and we assume the values $\mu$ are given as input to the system. 
%
The goal of the system is to produce a ranked list of items for each of the $n$ users. %Formally, for all $i \in \intint{n},$ the recommender system outputs $\sigma_i, $ a permutation of $\intint{m}$, such that $\sigma_i(j)$ is the rank of item $j$ in the list shown to user $i.$ 
Following previous work on fair rankings \citep[e.g.][]{singh2018fairness}, we consider randomized rankings because they enable the use of convex optimization techniques to generate the recommendations, which would otherwise involve an intractable combinatorial optimization problem in the space of all user's rankings. A randomized ranking for user $i$ is represented by a bistochastic matrix $\rrk_i \in \reals^{m\times m},$ where $\rrk_{ijk}$ is the probability that item $j$ is recommended to user $i$ at position $k.$ The recommender system is characterized by a \emph{ranking policy} $\rrk = (\rrk_i)_{i=1}^n$. We denote the convex set of ranking policies by $\rrkS$.

We use the term \emph{utility} in its broad sense in cardinal welfare economics as a ``\emph{measurement of the higher-order characteristic that is relevant to the particular distributive justice problem at hand}'' \citep{moulin2003fair}. Similarly to \cite{patro2020fairrec,wang2020fairness,do2021two}, we define the utility of a user as the ranking performance, and the utility of an item as its average exposure to users, which are formalized in \eqref{eq:utilities} below. Utilities are defined according to the position-based model \citep{biega2018equity,morik2020controlling,do2021two} with weights $\ew \in \reals_+^m$. The weight $\ew_k$ is the probability that a user examines the item at position $k$, and we assume that the weights are non-increasing. Since there are $K$ recommendation slots, we have $\ew_1 \geq \ldots \geq \ew_K$ and $\ew_k = 0$ for any $k > K$. The user and item utilities are then:
\begin{align}\label{eq:utilities}
    \hspace{-1.5em}\resizebox{0.92\linewidth}{!}{$\displaystyle\textit{User utility: }\, u_i(P) = \sum_{j=1}^m \muij \rrk_{ij}^\top \ew \quad\quad\textit{Item exposure: }\, v_j(P) = \sum_{i=1}^n\rrk_{ij}^\top \ew.$}
\end{align}
We follow a general framework where the ranking policy $\rrk$ is found by maximizing a global \emph{welfare function} $F(\rrk)$, and the welfare function is a weighted sum of welfare functions for users and items:
\begin{align}\label{eq:welfobj}
    \welfobj(\rrk) = (1-\lambda) \welfobjuser(\bu(\rrk)) + \lambda \welfobjitem(\bv(\rrk)),
\end{align}
where $\welfobjuser:\Re^n\rightarrow\Re$ and $\welfobjitem:\Re^m\rightarrow\Re$ respectively aggregate the utilities of users and item exposures and $\lambda\in[0,1]$ specifies the relative weight of users and items. 

\subsection{Generalized Gini welfare functions}

In this work, we focus on the case where $\welfobjitem$ and $\welfobjuser$ are based on Generalized Gini welfare functions (GGFs, \citep{weymark1981generalized}). A GGF $\giniwelf{\bw}:\Re^n\rightarrow \Re$ is a function parameterized by a vector $\bw \in \reals^n$ of non-increasing positive weights such that $\bw_1=1\geq\ldots\geq \bw_n\geq0$, defined a weighted sum of its sorted inputs, which is also called an ordered weighted averaging operator (OWA, \citep{yager1988ordered}). Formally, let $\bx\in\Re^n$ be a utility vector and denote by $\bx\sort$ the values of $\bx$ sorted in increasing order, i.e., $\bx_1\sort \leq ...\leq \bx_n\sort$. Then:
\begin{align}\label{eq:def:ggf}
    \giniwelf{\bw}(\bx) 
    %= \sum_{i=1}^n (\bw_{i}-\bw_{i+1}) \bxcum_i 
    = \sum_{i=1}^{n}\bw_i \bx_i\sort.
\end{align}
With non-increasing, non-negative $\bw$, it is well-known that OWA operators are concave \citep{yager1988ordered}. %\citep{fryer2005affirmative}.
This implies that the maximization of  \eqref{eq:welfobj} where both $\welfobjuser$ and $\welfobjitem$ are GGFs is a convex optimization problem (maximization of a concave function over the convex set of ranking policies). GGFs address fairness from the point of view of distributive justice in welfare economics \citep{moulin2003fair}, because they assign more weight to the portions of the population that have the least utility. Compared to a standard average, a GGF thus promotes more equality between individuals.

An alternative formula for $\giniwelf{\bw}(\bx)$ is based on the generalized Lorenz curve\footnote{Lorenz curves are normalized so that the last value is $1$, while generalized Lorenz curves are not normalized.} \citep{shorrocks1983ranking} of $\bx$, which is denoted $\bxcum$ and is defined as the vector of cumulative sums of sorted utilities:
\begin{align}
    \label{eq:def:ggfaslorenz}
    \giniwelf{\bw}(\bx) 
    = \sum_{i=1}^n (\bw_{i}-\bw_{i+1}) \bxcum_i
    &&
    \text{with~} \bxcum_i=\bx_1\sort+\ldots\bx_i\sort.
\end{align}
We used the convention $\bw_{n+1}=0$. Notice that since the weights $\bw$ are non-increasing,  we have that $\bw_{i}-\bw_{i+1}\geq 0$. This formula offers an alternative way of parametrizing GGFs in terms of fractions owned by quantiles of the population, which we use later. 

\paragraph{Relationship to the Gini index}
GGFs are welfare functions so they follow the convention that they should be maximized. Moreover, if $\bw_i>0$ for all $i$,  $\giniwelf{\bw}$ is increasing with respect to every individual utilities, which ensures that maximizers of GGFs are Pareto-optimal \citep{moulin2003fair}. The Gini index of $\bx$, denoted $\gini(\bx)$ is associated to the GGF with $\bw_i=\nicefrac{n-i+1}{n}$ \citep[for formulas of Gini index, see][]{yitzhaki2013more}:
\begin{align}\label{eq:def:giniindex}
    \gini(\bx)
    &= 1-\frac{2}{\norm{\bx}_1}\sum_{i=1}^n \frac{n-i+1}{n} \bx_i\sort\\
    &= \frac{1}{n^2\bxm}\sum_{i=1}^n\sum_{j=1}^n |\bx_i-\bx_j|
    && \text{with~} \bxm=\frac{1}{n}\sum_{i=1}^n \bx_i.
\end{align}
The second equality gives a more intuitive formula as a normalized average of absolute pairwise differences. The Gini index is an inequality measure, and therefore should be minimized, but, more importantly, it is normalized by the sum of utilities $\norm{\bx}_1$, which means that in general minimizing the Gini index does not yeild Pareto-optimal solutions. The importance of this normalization is discussed by e.g., \citep{atkinson1970measurement}, and by \citet{do2021two} in the context of fairness in rankings. Yet, when $\bx$ is a vector of item exposures $\bx=\bv(\rrk)$, the normalization is not important because the total exposure is constant. It is then equivalent to minimize the Gini index of item exposures or to maximize its associated GGF.

\subsection{GGFs for fairness in rankings} \label{sec:fairnesstasks}

As GGFs allow for arbitrary (non-negative) weights to each fraction of the population, it is a  flexible family of objective functions to define the normative fairness criterion. We give here some examples related to the existing literature on fairness in rankings.

\paragraph{Trade-offs between user utility and inequalities in item exposure} The first task consists in mitigating inequalities of exposure between (groups of) items, and appears in many studies \citep{singh2018fairness,zehlike2020reducing,wu2021tfrom}. This leads to a tradeoff between the total utility of users and inequalities among items, and such inequalities are usually measured by the Gini index (as in \citep{morik2020controlling,biega2018equity}). Removing the dependency on $\rrk$ to lighten the notation, a natural formulation of this trade-off uses the welfare function \eqref{eq:welfobj} with
\begin{align}\label{eq:def:eqexposure}
    % \hspace{-1em}\resizebox{0.92\linewidth}{!}{$
    \displaystyle\welfobjuser(\bu)=\frac{1}{n}\sum_{i=1}^n\bu_i
    \quad\quad
    \welfobjitem(\bv)
    =\sum_{i=1}^n \frac{n-i+1}{n} \bv_i\sort.
    % $}
\end{align}
As stated in the previous section, for item exposure, $\welfobjitem$ is equivalent to the Gini index. The Gini index for $\welfobjitem$ has been routinely used for \emph{evaluating} inequalities in item exposure \citep{morik2020controlling,biega2018equity} but there is no algorithm to optimize general trade-offs between user utility and the Gini index of exposure. \citet{morik2020controlling} use the Gini index of exposures in the context of dynamic ranking (with the absolute pairwise differences formula \eqref{eq:def:giniindex}), where their algorithm is shown to asymptotically drive $\welfobjitem(\bv)$ to $0$, equivalent to $\lambda\to 1$ in \eqref{eq:welfobj}. However, their algorithm cannot be used to converge to the optimal rankings for other values of $\lambda$. \citet{do2021two} use as baseline a variant using the standard deviation of exposures instead of absolute pairwise difference because it is easier to optimize (it is smooth except on $0$). Our approach allows for the direct optimization of \eqref{eq:welfobj} using the (desired) Gini index to measure inequalities between item exposures.

Note that several authors \citep{morik2020controlling,biega2018equity} used \emph{quality-weighted} exposure $\bv'_j(\rrk) = \bv(\rrk)/\overline{\mu}_j$ where $\overline{\mu}_j=\frac{1}{n}\sum_{i=1}^n\muij$ is the average value of item $j$ across users, rather than the exposure itself. We keep the non-weighted exposure to simplify the exposition, but our method straightforwardly applies to quality-weighted exposure.

\paragraph{The welfare approach to two-sided fairness} \citet{do2021two} view fairness in ranking from the perspective of distributive justice in welfare economics, in which the goal is to trade-off between total user utility and the utility of the worse-off fractions of the population. This leads to policies where exposure for the most popular items is ``redistributed'' to less popular items, leading to more equality of exposure for item fairness. Similarly, for user fairness, policies should make sure the worse-off users do not bear the cost of more equality of exposure between items. 

Formally, let $\phi(x, \alpha)=x^\alpha$ if $\alpha>0$, $\phi(x, \alpha)=\log(x)$ if $\alpha=0$ and $\phi(x, \alpha)=-x^\alpha$ if $\alpha<0$. \citet{do2021two} propose to use concave welfare functions of the form:
\begin{align}\label{eq:def-qua}
    \welfobjuser(\bu) = \sum_{i=1}^n \phi(\bu_i, \alpha_1) 
    &&
    \welfobjitem(\bv) = \sum_{j=1}^m \phi(\bv_j, \alpha_2)
\end{align}
Where $\alpha_1$ (resp. $\alpha_2$) is the hyperparameter that describes how much the rankings should redistribute utility on the user (resp. item) side. \citet{do2021two} motivate the choice of additively separable welfare functions \eqref{eq:def-qua} by their usage in cardinal welfare economics \citep{dalton1920measurement,atkinson1970measurement,shorrocks1980class,cowell1988inequality}. Yet, their experimental evaluation for user fairness relies on comparing trade-offs defined by the specific points of the Lorenz curve because it is easier to interpret than the values of $\alpha_1$. Our approach allows for the direct optimization of these evaluation criteria.

More generally, their fairness criterion, which is based on the comparison of generalized Lorenz curves of user utility and item exposure, allows for other rankings than what can be generated by the family of additively separable welfare functions \eqref{eq:def-qua}. As we see in the next subsection, the GGFs we optimize allow to generate \emph{every} ranking policy that \citet{do2021two} consider fair, and \emph{only} those. 

\subsection{Generating all Lorenz efficient solutions}

In welfare economics, the fundamental property of concave welfare functions is that they are monotonic with respect to the dominance of generalized Lorenz curves \citep{atkinson1970measurement,shorrocks1983ranking,moulin2003fair}, because this garantees that maximizing a welfare function performs an optimal redistribution from the better-off to the worse-off at every level of average utility. In the context of two-sided fairness in rankings, \citet{do2021two} formalize their fairness criterion by stating that a ranking policy is fair as long as the generalized Lorenz curves of users and items are not jointly dominated. In this section, we show that the family of GGFs allows to generate \emph{every} ranking policy that \citet{do2021two} consider fair, and \emph{only} those. The result follows from standard results of convex multi-objective optimization \citep{geoffrion1968proper,miettinen2012nonlinear}. We give here the formal statements for exhaustivity.

Let $\bx$ and $\bx'$ two vectors in $\Re_+^n$. We say that $\bx$ weakly-Lorenz-dominates $\bx'$, denoted $\bx\lorenzw\bx'$, when the generalized Lorenz curve of $\bx$ is always at least equal to that of $\bx'$, i.e., $\bx\lorenzw\bx' \iff \forall i, \bxcum_i \geq \bxcum_i'$. We say that $\bx$ Lorenz-dominates $\bx'$, denoted $\bx\lorenz\bx'$ if $\bx\lorenzw\bx'$ and $\bx\neq\bx'$, i.e., if the generalized Lorenz curve of $\bx$ is strictly larger than that of $\bx'$ on at least one point. The criterion that generalized Lorenz curves of users and items are not jointly-dominated is captured by the notion of \emph{Lorenz-efficiency}:
\begin{definition}[\citet{do2021two}]
A ranking policy $\rrk \in \rrkS$ is \emph{Lorenz-efficient} if there is no $\rrk' \in \rrkS$ such that either ($\bu(\rrk') \lorenzw\bu(\rrk)$ and $\bv(\rrk') \lorenz\bv(\rrk)$) or ($\bv(\rrk') \lorenzw\bv(\rrk)$ and $\bu(\rrk') \lorenz\bu(\rrk)$).
\end{definition}
Let $\wS_n = \{\bw \in \reals^n:  \bw_1=1 \geq \ldots \geq \bw_n \geq 0\}$ be the set of admissible weights of GGFs. Given $\ubw\in\wS_n$, $\ibw\in\wS_m$ and $\lambda \in(0,1)$, we define the \emph{two-sided GGF welfare function} as the welfare function \eqref{eq:welfobj} with $\welfobjuser = \giniwelf{\ubw}$ and $\welfobjitem=\giniwelf{\ibw}$:
\begin{align}\label{eq:def-2sidedggf}
    \welfobj_{\lambda, \ubw, \ibw}(\rrk) = (1-\lambda)\giniwelf{\ubw}\big(\bu(\rrk)\big) + \lambda \giniwelf{\ibw}\big((\bv(\rrk)\big).
\end{align}
% which is the welfare function 
% Then:
\begin{proposition}\label{lem:all-lorenz} Let $\Theta=(0,1)\times\wS_n\times\wS_m$.
    \begin{enumerate}
        \item Let $(\lambda, \ubw, \ibw)\in\Theta$, where $\ubw$ and $\ibw$ have strictly decreasing weights, and $\rrk^* \in \argmax_{\rrk\in\rrkS}\welfobj_{\lambda, \ubw, \ibw}(\rrk)$. 
        
        Then $\rrk^*$ is Lorenz-efficient. 
        \item If $\rrk$ is Lorenz efficient, then there exists $(\iw,\ubw,\ibw) \in \Theta$ such that $\rrk\in\argmax_{\rrk \in \rrkS} \welfobj_{\lambda, \ubw, \ibw}(\rrk)$.
    \end{enumerate}
\end{proposition}
\begin{proof}
The proof uses standard results on convex multi-objective optimization from \citep{geoffrion1968proper,miettinen2012nonlinear}. The GGFs corresponds to the scalarization of the multi-objective problem of jointly maximizing the generalized Lorenz curves of users and items, which is a multi-objective problems with $n+m$ objectives (one objective for each point of the curve). The result follows from the observation that the Lorenz-efficiency of $\rrk$ is equivalent to Pareto-efficiency of the set of points of the Lorenz-curves of users and items.

Indeed, we are optimizing over the convex set of stochastic ranking policies, and each objective function is concave because it corresponds to an OWA operator with non-increasing weight applied to utilities or exposures, which are linear functions of the ranking policy. The multi-objective problem is then concave, which means that the maximizers of all weighted sums of the objective with strictly positive weights are Pareto-efficient. Reciprocally every Pareto-efficient solution is a solution of one positive weighted sum of the objectives. 
\end{proof}




==> sections/old/introduction.tex <==
\section{Introduction} \label{sec:intro}

Recommender systems play an important role in organizing the information available to us, by deciding on which content should be exposed to users and how it should be prioritized. These decisions impact both the users and the item producers of the platform. While recommender systems are usually designed to maximize performance metrics of user satisfaction, several audits recently revealed potential performance disparities across users \citep{sweeney2013discrimination,datta2015automated,ekstrand2018all,mehrotra2017auditing}. On the side of item producers, the growing literature on fairness of exposure aims to avoid popularity biases \citep{abdollahpouri2019unfairness} by reducing inequalities in the exposure of different items \citep{singh2018fairness}, or aiming for equal exposure weighted by relevance \citep{diaz2020evaluating,biega2018equity,morik2020controlling}. In most cases, the approaches proposed for user-side and item-side fairness aim to reduce inequalities, a goal which is well studied in the literature on inequality measurement in economics \citep{cowell1988inequality}, and for which the most well-known measure is the Gini index \citep{gini1921measurement}.


Generalized Gini welfare Functions (GGFs, \citep{weymark1981generalized}) are used in the domain of cardinal welfare economics \citep{moulin2003fair} to make decisions by maximizing a weighted sum of the utilities of individuals, where the weight attached to an individual depends on the rank of its utility in the population. Giving more weight to individuals with lower ranks gives more importance to worse-off people, hence promoting more equality.  GGFs include the well-known Gini index as a special case. For fairness in recommender systems, they  can therefore be used to maximize average user utility while minimizing inequalities of item exposure, where inequality is measured by the Gini index. GGFs also conveniently specify normative criteria based on utility quantiles, which are easy to interpret. As a multi-objective optimization method, we show that varying the weights of GGFs allow to generate all ranking policies with non-dominated generalized Lorenz curves, a fairness property recently studied in two-sided fairness for recommender systems under the name of Lorenz efficiency \citep{do2021two}. 

The difficulty of using GGFs as objective functions for fairness in ranking stems from their non-differentiability, which leads to computational challenges. Indeed, ranking with fairness of exposure requires the solution of a global optimization problem in the space of (randomized) rankings of all users, because the exposure of an item is the sum of its exposure to each individual users. Even though many objective functions of interest are concave, the only scalable approach known to date \citep{do2021two} uses the Frank-Wolfe algorithm \citep{frank1956algorithm}. However, the convergence of vanilla Frank-Wolfe algorithms requires a bounded curvature of the objective function \citep{clarkson2010coresets,nesterov2018complexity} -- in essence, bounded second-order derivatives -- a property that GGFs do not satisfy because they are non-differentiable. Approaches to optimizing GGFs outside the field of ranking, using the linearization of ordered weighted averages \citep{ogryczak2003solving} or online subgradient descent \citep{busa2017multi} require dense updates in the space of randomized ranking policies, which are prohibitively expensive in the case of ranking. Frank-Wolfe algorithms naturally make sparse updates \citep{clarkson2010coresets,jaggi2013revisiting}, which is why they are particularly suited to structured prediction problems \citep{lacoste2013block}.

We propose a new approach to the optimization of GGFs based on extensions of Frank-Wolfe algorithms for non-smooth optimization \citep{lan2013complexity,yurtsever2018conditional,2020thekumparampil}, which are based on optimizing smoothed surrogate objective functions, with a smoothing parameter that converges to $0$. A common smoothing technique uses the Moreau envelope, and our main insight is that the gradient of the Moreau envelope of GGFs can be computed in $O(n \log n)$ operations, where $n$ is the number of users or items. This result unlocks the use of Frank-Wolfe algorithms with GGFs, allowing us to efficiently find optimal ranking policies while optimizing GGFs. 

We showcase the performances of the algorithm on two recommendations tasks of movies and music, and on a reciprocal recommendation problem (such as dating, where users are recommended to other users), with datasets involving up to $15k$ users and items. Compared to relevant baselines, we show that our algorithm successfully yields better trade-offs in terms of user utility and exposure in item inequality measured by the Gini index. Our approach also successfully finds better trade-offs in terms of two-sided fairness when maximizing the lower quantiles of user utility while minimizing the Gini index of item exposure.

In the remainder of the paper, we first describe our recommendation framework. We then present the family of generalized Gini welfare functions and its relationship to previously proposed fairness criteria in ranking. In Sec.~\ref{sec:moreau-ggf} we provide the details of our algorithm and the convergence guarantees. Our experimental results are reported in Sec.~\ref{sec:xps}, and an extension to reciprocal recommendation problems is discussed in Sec.~\ref{sec:reciprocal}. We position our approach with respect to the related work in Sec.~\ref{sec:related}, and Sec.~\ref{sec:conclu} concludes the paper and discusses the limitations of our work.

% \nico{remember to put that somewhere (if we really need that, it seems to me that we don't}
% \paragraph{Notation} 
% Given a vector $\bz\in\Re^n$, let $\bzsort$ be the vector of values of $\bz$ sorted increasing order, i.e., $\bzsort_1 \leq \ldots \leq \bzsort_n$, then the generalized Lorenz curve of $\bz$ is $\bzcum = (\bzcum_i)_{i=1}^n$ where $\bzcum_i = \bzsort_1+\ldots+\bzsort_i$. 

% \nico{maybe clean or remove this notation part -- what do we really need?}\nico{should we define the notation for the dot product?}\nico{We should probably say that vectors are in bold and we "de-bold" when we take the subscript}

==> sections/old/moreau.tex <==
\section{Optimizing Generalized Gini Welfare} \label{sec:moreau-ggf}

In this section. we provide a scalable method for optimizing two-sided GGFs welfarefunctions \eqref{eq:def-2sidedggf}. The challenge of optimizing GGFs is that they are nondifferentiable since they require sorting utilities. We first describe why existing approaches to optimize GGFs are not suited to ranking in Sec.~\ref{sec:algo-challenge}. We then show how to compute the gradient of the Moreau envelope of GGFs in Sec.~\ref{sec:algo-gradient} and present the full algorithm in Sec.~\ref{sec:algo-algo}.


\subsection{Challenges} \label{sec:algo-challenge}

In multi-objective optimization, a standard approach to optimizing OWAs is to solve the equivalent linear program derived by \citet{ogryczak2003solving}. Because the utilities depend on 3d-tensors $\rrk \in \rrkS$ in our case, the linear program has $O(n \cdot m^2)$ variables and constraints, which is prohibitively large in practice. 

Another approach consists in using subgradients to optimize GGFs, like \citet{busa2017multi}. A subgradient of $g_{\bw}$ in $\bz$ is given by $\xvector{w_{\sigma^{-1}}},$ where $\sigma \in \argsort\sort(\bz).$ Gradient descent algorithms are robust to subgradients \citep{shamir2013stochastic}, but using them would require to project iterates onto the solution space, which in our case involves costly projections onto the space of stochastic ranking policies $\rrkS.$ 

On the other hand, the Frank-Wolfe algorithm \citep{frank1956algorithm} was shown to provide a computationally efficient and provably convergent method to optimize over $\rrkS$ \citep{do2021two}. However, it only applies to smooth functions, and  
replacing gradients with subgradients in Frank-Wolfe does not guarantee convergence \citep{nesterov2018complexity}. 

We turn to Frank-Wolfe variants for nonsmooth objectives, since Frank-Wolfe methods are well-suited to our structured ranking problem \citep{do2021two}. More precisely, following \citep{lan2013complexity,yurtsever2018conditional,2020thekumparampil}, our algorithm uses the Moreau envelope of GGFs for smoothing. The usefulness of this smooth approximation depends on its gradient, which computation is in some cases intractable \citep{chen2012smoothing}. Our main technical contribution is to show that the gradient of the Moreau envelope of GGFs can be computed in $O(n \log n)$ operations.

\subsection{The Moreau envelope of GGFs}\label{sec:algo-gradient}


\paragraph{Notation} $\norm{\bz} = \sqrt{\sum_{i=1}^n (z_i)^2 }$ denotes the $\ell_2$ norm. The projection onto a compact convex $\mathcal{X}$ is denoted by $\proj_{\mathcal{X}}(\bz):= \argmin\limits_{\bz' \in \mathcal{X}}\norm{\bz - \bz'}^2.$ $D_\mathcal{X} := \max\limits_{\bz, \bz' \in \mathcal{X}}\|\bz - \bz'\|$ is the diameter of $\mathcal{X}.$
Given an integer $n \in \mathbb{N},$ $\intint{n} := \{1,\ldots,n\}\,$, and $\permSn$ denotes the set of permutations of $\intint{n}.$ Given $\bz \in \reals^n$, $\argsort\sort(\bz) = \{\sigma\in \permSn: z_{\sigma(1)} \leq\ldots\leq z_{\sigma(n)}\}$ sorts $\bz$ in increasing order, and $\argsort\descsort$ decreasingly. Let $\topk(\bz) = \{ \sigma \in \permSn: z_{\sigma(1)}\geq \ldots \geq z_{\sigma(K)} \text{ and } \forall k\geq K, z_{\sigma(K)} \geq z_k\}$ be a ranked list of the $k$-largest elements in $\bz$.

\subsubsection{Definition and properties} Let us fix weights $\bw \in \wS$ and focus on maximizing the GGF $g_{\bw}.$ We introduce $h(\bz) := -g_{\bw}(\bz)$ and $f(P) = h(\bu(P))$ 
to obtain a convex minimization problem: $\min\limits_{P \in \rrkS} f(P)$. We notice that $h$ is $\|\bw\|$-Lipschitz continuous, and that: $~h(\bz) = -\min\limits_{\sigma \in \permSn} \bwsigt \bz = \max\limits_{\sigma \in \permSn } -\bwsigt \bz.$

\begin{definition}[Smoothness]
A function $L: \mathcal{X}\subseteq \reals^n \rightarrow \reals$ is said to be $C$-smooth if it is differentiable and if its gradient is $C$-Lipschitz continuous, i.e., if $\forall \bx,\bx' \in \mathcal{X}\,, \norm{\nabla L(\bx) - \nabla L(\bx')} \leq C \norm{\bx - \bx'}.$
\end{definition}

% We consider the smooth approximation\footnote{It is also equal to the Moreau envelope of $h$, by strong duality.} of $h$ from \citet{nesterov2005smooth}, defined as: 
% \begin{equation}
%     \hbeta(\bz) = \max_{\by \in \reals^n} \xdp{\bz}{\by} - h^*(\by) - \frac{\beta}{2}\|\by\|,
% \end{equation} for some smoothing parameter $\beta > 0$.  The proximal operator is defined as $\prox_{\phi}(\bz) = \argmin _{\bz' \in \mathcal{U}} \phi(\bz) + \frac{1}{2}\|\bz'-\bz\|^2.$


We consider the smooth approximation of $h$ given by its Moreau envelope\footnote{By the Fenchel duality theorem \citep{rockafellar2015convex}, it is also equal to the smoothing technique of \citet{nesterov2005smooth} with the Euclidean proximity function $\frac{1}{2} \norm{\cdot}^2$, which is the dual formulation of the Moreau envelope (see \citep[Sec. 4.3]{beck2012smoothing}).} , defined as:
\begin{align}
    h^\beta(\bz) = \min_{\bz' \in \US} h(\bz') + \frac{1}{2 \beta} \norm{\bz - \bz'}^2.
\end{align}
$h^\beta$ is known to be $\frac{1}{\beta}$-smooth \citep{parikh2014proximal}. The parameter $\beta$ controls the trade-off between the smoothness of $\hbeta$ and the quality of its approximation of $h.$ We also introduce $\fbeta = \hbeta \circ u.$



\subsubsection{Efficient computation of the gradient} \label{sec:isotonic}



\begin{algorithm}
    \caption{\label{alg:grad-moreau} Computation of $\nabla \fbeta(\rrk)$}
    \DontPrintSemicolon
     \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
     
     \Input{values $\muij$, ranking $\rrk$, smoothing $\sm$, GGF weights $\bw$}
     \Output{$\nabla \fbeta(P)$}
     $\bw \gets -(\bw_n,...,\bw_1)$, $\bz \gets \frac{\bu(\rrk)}{\beta}~$ and      $\pi \gets \argsort\descsort(\bz)~$\;
     $\bx \gets \PAV(\bz_{\pi} - \bw)~$\;
     $\by\gets \bz + \xvector{x_{\pi^{-1}}}$\;
     Return $\left(y_i \muij \ew_k\right)_{i,j,k}$.
\end{algorithm}

We now present our main technical contribution, which is an efficient procedure for the computation of the Moreau envelope's gradient. For $\bx \in \reals^n$, let $\ph(\bx)$ denote the permutahedron induced by $\bx$, defined as the convex hull of all permutations of the vector $\bx$: $\,\ph(\bx) = \conv\{\bxsig : \sigma \in \permSn\}.\,$ The following proposition formulates $\nabla \fbeta$ as a projection onto a permutahedron:

\begin{proposition}\label{prop:grad-moreau}

Let $\tbw = -(w_n,...,w_1)$. Let $\rrk \in \rrkS$ and $\projbetaP = \proj_{\ph(\tbw)}\left(\frac{\bu(P)}{\beta}\right).$ Then for all $(i,j,k) \in \intint{n} \times \intint{m}^2$, we have:
\begin{equation}
\begin{aligned}\label{eq:grad-moreau} 
    \frac{\partial \fbeta}{\partial P_{ijk}}(P) = \projbetaPi \muij \ew_k.
\end{aligned}
\end{equation}
\end{proposition}

\begin{proof} The proximal operator is defined as $\prox_{\phi}(\bz) = \argmin\limits_{\bz' \in \mathcal{U}} \phi(\bz) + \frac{1}{2}\|\bz'-\bz\|^2.$ We remind that the gradient of $\fbeta = \hbeta \circ u$ is given by: $\grad \fbeta(P) = \frac{1}{\beta} \bu^* (\bu(P) - \prox_{\beta h}(\bu(P)),$  where $\bu*$ is the adjoint of $\bu$ (see \citep[e.g.][]{parikh2014proximal}).

$h$ can be written as the support function of the convex $\ph(\tbw)$, where $\tbw = -(w_n,...,w_1)$, since:
\begin{align*}
    h(\bz) = \max_{\sigma \in \permSn} -\bwsigt \bz = \sup_{\by \in \ph(\tbw)} \by^\intercal \bz.
\end{align*}
Then the Fenchel conjugate of $h$ is known to be the indicator function of the convex $\ph(\tbw)$, and its proximal is the projection $\proj_{\ph(\tbw)}$ \citep{parikh2014proximal}. By Moreau decomposition, we get: $~\prox_{\beta h}(\bz) = \bz - \beta \proj_{\ph(\tbw)}\left(\nicefrac{\bz}{\beta}\right),$ and thus:
\begin{equation}
\begin{aligned}\label{eq:yt-proj}
    \grad \fbeta(P) = \bu^* \left(\proj_{\ph(\tbw)}\left(\nicefrac{\bu(P)}{\beta}\right)\right).
\end{aligned}
\end{equation}
The result follows from the definition of $\bu$ as $\bu: P \mapsto \sum_{j,k} \muij P_{ijk} \ew_k.$
\end{proof}


% The parameter $\beta$ controls the trade-off between the smoothness of $\fbeta$ and the quality of its approximation of $f.$ We note that $\beta \rightarrow 0, $ $\grad \fbeta$ converges to a subgradient of $f$ in $P.$
% \begin{corollary}\label{cor:subgradient} Let $\rrk \in \rrkS$ and $\sigma \in \argsort\sort(\bu(P)).$ Then:
% \begin{align}\label{eq:subgradient}
%     \frac{\partial \fbeta}{\partial P_{ijk}}(P) \xrightarrow[\beta \rightarrow 0]{} \bw_{\sigma^{-1}(i)} \muij \ew_k,
% \end{align}
% which is a subgradient of $f$ in P.
% \end{corollary}


Overall, computing the gradient of the Moreau envelope boils down to a projection onto the permutahedron $\ph(\tbw)$. This projection was shown by several authors to be reducible to isotonic regression:
\begin{proposition}[Reduction to isotonic regression \citep{negrinho2014orbit,lim2016efficient,blondel2020fast}]\label{prop:isoto} Let $\sigma\in\permSn$ that sorts $\bz$ decreasingly, i.e. $z_{\sigma(1)} \geq \ldots \geq z_{\sigma(n)}.$
Let $\bx$ be a solution to isotonic regression on $\bzsig - \tbw$, i.e.
\begin{align}
    \bx = \argmin_{x'_1 \leq \ldots \leq x'_n} \frac{1}{2}\|\bx' - (\bzsig - \tbw)\|^2
\end{align}
Then we have: $ \proj_{\ph(\tbw)}(\bz) = \bz + \xvector{x_{\sigma^{-1}}}.$
\end{proposition}

Following these works, we use the Pool Adjacent Violators (\PAV) algorithm for isotonic regression, which was shown to output an exact solution in $O(n)$ iterations given a sorted input \cite{best2000minimizing}. 

The algorithm for computing $\nabla \fbeta(P)$ is summarized in Alg. \ref{alg:grad-moreau}. Including the sorting of $\frac{\bu(P)}{\beta}$, it costs $O(n \log n)$ time and $O(n)$ space. 

% \nico{After the proof (or at the beginning of the section, where you explain the pieces you bring together, I think it's worthwhile to mention the relationship and differences with differentiable sorting and Blondel et. al, because it feels this is timely work and it (may) increase the perception that what you say here is not well-known.}

\begin{remark}\label{rk:blondel}
Our method is related to the differentiable sorting operator of \citet{blondel2020fast}, which uses a regularization term to smooth the linear formulation of sorting. The regularized form can itself be written as a projection to a permutahedron. In our case, this projection appears in the gradient of the GGF, rather than the GGF itself. This is important because the form of $\grad \fbeta (P)$ given by Prop. \ref{prop:grad-moreau} as an outer product with $(\ew_k)_k$ unlocks the result of Prop. \ref{prop:fwgrad} in the following subsection. This is the key to fast Frank-Wolfe iterations in our optimization problem over stochastic ranking policies.
\end{remark}




\subsection{Frank-Wolfe with smoothing}\label{sec:algo-algo}

We return to our two-sided GGF objective \eqref{eq:def-2sidedggf}, and from now on we fix the parameters $(\iw,\ubw,\ibw)$ and consider the minimization of $f := -F_{\iw,\ubw,\ibw}$ over $\rrkS.$ Since there is a GGF for users and a GGF for items, for $\beta > 0$ we denote by $h_1^\beta$ and $h_2^\beta$ the respective Moreau envelopes of $-\uGGF$ and $-\iGGF.$ We also denote by $\fbeta$ the smooth approximation of $f$:
\begin{align}\label{eq:2sided-moreau}
    \fbeta(P) := (1-\iw) h_1^\beta(\bu(P)) + \iw h_2^\beta(\bv(P)).
\end{align}

Our algorithm \fwsmooth (Alg. \ref{alg:nonsmoothfw}) for minimizing $f$ uses the Frank-Wolfe method for nonsmooth optimization from \citet{lan2013complexity}. It constructs iterates $P^{(t)}$ , and given a positive sequence $(\beta_t)_{t\geq 1}$ decreasing to $0$, at each iteration $t$, the algorithm applies Frank-Wolfe updates to the smooth approximation $\fbetat.$ More precisely, \fwsmooth takes a direction search step with respect
to the $\grad \fbetat$ of $f$, by calculating:
\begin{align}\label{eq:fw-step}
    &\Qt = \argmin_{\rrk\in\rrkS} \xdp{\rrk}{\grad \fbetat(P^{(t)})}.
\end{align}

% \begin{algorithm}
%     \caption{\label{alg:nonsmoothfw}\fwsmooth}
%     \DontPrintSemicolon
%      \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
     
%      \Input{values $(\mu_{ij})$, $\#$ of iterations $T$, smoothing seq. $(\beta_t)_{t}$}
%      \Output{ranking policy $\rrk^{(T)}$}
     
%      Let $\rrk^{(0)}$ be the utilitarian ranking policy\;
%      \For{t=1, \ldots, T}{
%      Compute $\grad \fbetat(P^{(t)})$ using Alg. \ref{alg:grad-moreau}\;
%      $\Qt \gets \argmin_{\rrk\in\rrkS} \xdp{\rrk}{\grad \fbetat(P^{(t)})}$ \tcp{$\topk({-\tilde{\mu_i}})$ of Prop. \ref{prop:fwgrad}}\;
%      $\rrk^{(t)} \gets (1-\frac{2}{t+2})\rrk^{(t-1)} + \frac{2}{t+2}\Qt\,$\;
%       }
%       Return $\rrk^{(T)}$.
% \end{algorithm}


\begin{algorithm}
    \caption{\label{alg:nonsmoothfw}\fwsmooth}
    \DontPrintSemicolon
     \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
     
     \Input{values $(\mu_{ij})$, $\#$ of iterations $T$, smoothing seq. $(\beta_t)_{t}$}
     \Output{ranking policy $\rrk^{(T)}$}
     
     Initialize $\rrk^{(0)}$ as the utilitarian ranking policy, i.e. such that $\rrk^{(0)}_i$ represents $\tilde{\sigma}_i \in \argsort\descsort(\mu_i).$\;
     \For{t=1, \ldots, T}{
     Compute $\grad \fbetat(P^{(t)})$ using Alg. \ref{alg:grad-moreau} (for each GGF).\;
     \For{i=1, \ldots, \n}{
          $\tempmuij \gets \frac{1}{\ew_k} \frac{\partial \fbetat}{\partial P_{ijk}}(\rrkt)$ \tcp{does not depend on $k$}\;
          $~~\tilde{\sigma}_i \gets \topk( -\tilde{\mu}_i )$ \tcp{ Direction step \eqref{eq:fw-step}}
          }
     Let $\Qt \in \rrkS$ such that $\Qt_i$ represents  $\tilde{\sigma}_i$\;
     $\rrk^{(t)} \gets (1- \frac{2}{t+2})\rrk^{(t-1)} +  \frac{2}{t+2}\Qt\,$.
     }
     Return $\rrk^{(T)}$.
\end{algorithm}


\paragraph{Efficient computation of the Frank-Wolfe direction step} Frank-Wolfe methods are advantageous when step \eqref{eq:fw-step} can be computed efficiently, which was shown to be the case for smooth ranking objectives \citep{do2021two}. Similarly to \citet{do2021two}, the form of $\grad \fbeta(P)$ given by our Proposition \ref{prop:grad-moreau} is an outer product with the nonincreasing exposure weights $\ew_k$, which enables to solve step \eqref{eq:fw-step} with only one top-$K$ sorting operation per user. 



\begin{proposition}\label{prop:fwgrad}
Let $\tilde{\mu} = \frac{1}{\ew} \otimes \grad \fbetat(\rrkt) \in \reals^{n\times m}.$ For all $i \in \intint{n},$ let $\tilde{\sigma}_i \in \topk(-\tilde{\mu}_i)$ and $\Qt_i$ a permutation matrix representing $\tilde{\sigma}_i$.
Then $\Qt \in \argmin\limits_{\rrk \in \rrkS} \xdp{\rrk}{\grad \fbetat(\rrkt)}.$
\end{proposition}


\begin{proof}
Using the expression of the gradient of the Moreau envelope derived in Proposition \ref{prop:grad-moreau}, eq. \eqref{eq:grad-moreau}, we have:\begin{align*}
        \frac{\partial \fbetat}{\partial P_{ijk}}(\rrkt) & = (1 - \iw)  \frac{\partial }{\partial P_{ijk}}(h_1^{\beta_t}(\bu(\rrkt)) + \iw  \frac{\partial }{\partial P_{ijk}}(h_1^{\beta_t}(\bv(\rrkt))   \\
        % & = (1 - \iw) \, \muij \ew_k (\proj_{\ph(\utbw)}\left(\nicefrac{\bu(P)}{\beta}\right))_i + \iw \, \ew_k (\proj_{\ph(\itbw)}\left(\nicefrac{\bv(P)}{\beta}\right))_j \\
        & = \tempmuij \times \ew_k,
\end{align*}
where $\tempmuij = (1 - \iw) \, \muij \proj_{\ph(\utbw)}\left(\nicefrac{\bu(\rrkt)}{\beta_t}\right)_i + \iw \, \proj_{\ph(\itbw)}\left(\nicefrac{\bv(\rrkt)}{\beta_t}\right)_j,$ and thus $\tilde{\mu} \in \reals^{n \times m}.$

The result follows from Lem. 3 of \citep{do2021two} and is a consequence of the rearrangement lemma \cite{hardy1952inequalities}: the optimal $\Qt \in \argmin\limits_{\rrk \in \rrkS} \xdp{\rrk}{\grad \fbetat(\rrkt)}$ is obtained by sorting $\tempmuij$ in increasing order (or equivalently, $-\tempmuij$ in decreasing order since we consider the minimization of $f=-F$).
\end{proof}




\paragraph{Algorithm and theoretical guarantees} Each iteration of FW-smoothing (Alg. \ref{alg:nonsmoothfw}) combines (Line 3) the computation of $\grad \fbetat(\rrkt)$ given by the subroutine Alg. \ref{alg:grad-moreau}, with (Lines 4-8) the computation of the Frank-Wolfe direction step \eqref{eq:fw-step} derived in Prop. \ref{prop:fwgrad}. 

To compute $\grad \fbetat(\rrkt)$ (Line 3), the routine Alg. \ref{alg:grad-moreau} must be applied twice, once for the gradient of $h_1^{\beta_t}$ and once for the gradient of $h_2^{\beta_t},$ and the outputs are weighted with $\iw$ as per eq. \eqref{eq:2sided-moreau}. For $\grad h_2^{\beta_t}$, we use $\muji$ values all equal to 1 as input to Alg. \ref{alg:grad-moreau}, since items have uniform preferences over users in this recommendation setting. 

Applying the convergence result of \citet{lan2013complexity}, we obtain\footnote{In more details, the convergence guarantee of \citet{lan2013complexity} uses the operator norm of $\bu$ and $\bv$, which we bound as follows: $\norm{u(P)}^2 \leq \sum_{i} \sum_{j,k} (\muij P_{ijk} \ew_k)^2 \leq \ew_1^2 \norm{P}^2$, because $\muij \in [0,1]$ $\ew_k \in [0,\ew_1],$ and similarly $\norm{\bv(P)}^2 \leq \ew_1^2 \norm{P}^2$}:

\begin{proposition}[Th. 4, \citep{lan2013complexity}]\label{prop:converge} With $\beta_0 = \frac{2 D_{\rrkS} \ew_1}{\|\bw\|} $ and $\beta_t = \frac{2}{\sqrt{t+1}}$, \fwsmooth obtains the following convergence rate: $$f(P^{(T)}) - f(P^*) \leq \frac{2 D_{\rrkS} \ew_1 \|\bw\|}{\sqrt{T+1}}.$$
\end{proposition}

Combining the complexity of Algorithm \ref{alg:grad-moreau} with the result of Proposition \ref{prop:fwgrad}, we obtain the following complexity result:

\begin{proposition}\label{prop:complexity} For each user, an iteration costs $O(n \ln n + m \ln m)$ operations and $O(n + m)$ memory. The total amount of storage required per user is $O(K T)$.
\end{proposition}

Moreover, the algorithm provides a \emph{sparse representation of the stochastic rankings} as a weighted sum of permutation matrices, since $\rrkt$ is updated using the linear combination of (Line 9, Alg. \ref{alg:nonsmoothfw}). In other words, this gives us a Birkhoff-von-Neumann decomposition \cite{birkhoff1940lattice} of the bistochastic matrices \emph{for free}, avoiding the overhead of an additional decomposition algorithm as in existing works on fair ranking \citep{singh2018fairness,wang2020fairness,su2021optimizing}. 


\virginie{todo: Add a sentence saying that we are able to do what people wanted to do, but did not know how to!}

==> sections/old/old_framework.tex <==
\newpage
\section{Fairness in recommender systems} \label{sec:fairranking}

\subsection{Recommendation framework}\label{sec:framework}

We consider a recommendation scenario with $n$ users, and $m$ items, and $K$ recommendation slots. $\mu_{ij} \in [0,1]$ denotes the value of item $j$ for user $i$ (e.g, a ``liking'' probability), and we assume the values $\mu$ are given as input to the recommender system. 

The goal of the system is to produce a ranked list of items for each of the $n$ users. %Formally, for all $i \in \intint{n},$ the recommender system outputs $\sigma_i, $ a permutation of $\intint{m}$, such that $\sigma_i(j)$ is the rank of item $j$ in the list shown to user $i.$ 
Following previous work on fair rankings \citep[e.g.][]{singh2018fairness}, we consider randomized rankings because they enable the use of convex optimization techniques to generate the recommendations, which would otherwise involve intractable combinatorial optimization problems in the space of all user's rankings. A randomized ranking for user $i$ is represented by a bistochastic matrix $\rrk_i \in \reals^{m\times m},$ where $\rrk_{ijk}$ is the probability that item $j$ is recommended to user $i$ at position $k.$ The recommender system is characterized by a \emph{ranking policy} $\rrk = (\rrk_i)_{i=1}^n$. We denote the convex set of stochastic ranking policies by $\rrkS$.

We use the term \emph{utility} in its broad sense in cardinal welfare economics as a ``\emph{measurement of the higher-order characteristic that is relevant to the particular distributive justice problem at hand}'' \citep{moulin2003fair}. Similarly to \citet{do2021two}, we define the utility of a user as the ranking performance, and the utility of an item as its average exposure to users, which are formalized in \eqref{eq:utilities} below. Utilities are defined according to the position-based model \citep{biega2018equity,morik2020controlling,do2021two} with weights $\ew \in \reals_+^m$. The weight $\ew_k$ is the probability that a user examines the item at position $k$, and we assume that the weights are non-increasing. Since there are $K$ recommendation slots, we have $\ew_1 \geq \ldots \geq \ew_K$ and $\ew_k = 0$ for any $k > K$. The user and item utilities are then:
\begin{align}\label{eq:utilities}
    \hspace{-1.5em}\resizebox{0.92\linewidth}{!}{$\displaystyle\textit{User utility: }\, u_i(P) = \sum_{j=1}^m \muij \rrk_{ij}^\top \ew \quad\quad\textit{Item exposure: }\, v_j(P) = \sum_{i=1}^n\rrk_{ij}^\top \ew.$}
\end{align}
We follow a general framework where the ranking policy $\rrk$ is found by maximizing a global \emph{welfare function} $F(\rrk)$, and the welfare function is a weighted sum of welfare functions for users and items:
\begin{align}\label{eq:welfobj}
    \welfobj(\rrk) = (1-\lambda) \welfobjuser(\bu(\rrk)) + \lambda \welfobjitem(\bv(\rrk)),
\end{align}
where $\welfobjuser:\Re^n\rightarrow\Re$ and $\welfobjitem:\Re^m\rightarrow\Re$ respectively aggregate the utilities of users and item exposures and $\lambda\in[0,1]$ specifies the relative weight of users and items. 

\subsection{Fairness in rankings}

In this work, we focus on the case where $\welfobjitem$ and $\welfobjuser$ are based on generalized Gini welfare functions, which we describe in the next section. We give here additional context to position our work.

There are two main approaches to fairness in rankings: maximizing average user utility while aiming at equal exposure \citep{morik2020controlling,biega2018equity}, or maximizing concave functions of the utlities \citep{do2021two}. In our framework, these are summarized by the following choices:
\paragraph{Equal exposure} A formulation of the equal exposure criterion is:
\begin{align}\label{eq:def:eqexposure}
    \hspace{-1em}\resizebox{0.92\linewidth}{!}{
    $\displaystyle\welfobjuser(\bu(\rrk))=\frac{1}{n}\sum_{i=1}^n\bu_i(\rrk)
    \quad\quad
    \welfobjitem(\bv(\rrk))
    =-\!\!
    \sum_{\substack{j=1..m\\j'=1..m}} \!\!\big|\bv_j(\rrk) - \bv_{j'}(\rrk)\big|
    $}
\end{align}
There is a minus sign in $\welfobjitem$ because the welfare is maximized. In this case, it corresponds to maximizing user utility while \emph{mimising} inequalities in item exposure. The formula above for $\welfobjitem$ was used by \citep{morik2020controlling} in the context of dynamic ranking, where their algorithm is shown to asymptotically drive $\welfobjitem(\bv(\rrk))$ to $0$, equivalent to $\lambda\to 1$ in \eqref{eq:welfobj}. However, their algorithm cannot be used to converge to the optimal rankings for other values of $\lambda$. \citet{do2021two} use as baseline a variant using the standard deviation of exposures instead of absolute pairwise difference because it is easier to optimize. As we see later, our approach allows for the optimization of \eqref{eq:welfobj} with the definitions in \eqref{eq:def:eqexposure} since $\welfobjitem$ is a Gini index.

Note that previous authors \citep{morik2020controlling,biega2018equity} used \emph{quality-weighted} exposure $\bv'_j(\rrk) = \bv(\rrk)/\overline{\mu}_j$ where $\overline{\mu}_j=\frac{1}{n}\sum_{i=1}^n\muij$ is the average value of item $j$ across users, rather than the exposure itself. We keep the non-weighted exposure to simplify the exposition, but our methods straightforwardly applies to quality-weighted exposure.

\paragraph{The welfare approach to two-sided fairness} \citet{do2021two} view fairness in ranking from the perspective of distributive justice in welfare economics, in which the goal is to trade-off between total user utility and the utility of the worse-off fractions of the population. This leads to policies where exposure for the most popular items is ``redistributed'' to less popular items, leading to more equality of exposure for item fairness. Similarly, for user fairness, policies should make sure the worse-off users do not bear the cost of more equality of exposure between items. 

Formally, let $\phi(x, \alpha)=x^\alpha$ if $\alpha>0$, $\phi(x, \alpha)=\log(x)$ if $\alpha=0$ and $\phi(x, \alpha)=-x^\alpha$ if $\alpha<0$. \citet{do2021two} propose to use concave welfare functions of the form:
\begin{align}\label{eq:def-welf}
    \welfobjuser = \sum_{i=1}^n \phi(u_i(P), \alpha_1) 
    &&
    \welfobjitem = \sum_{j=1}^m \phi(v_j(P), \alpha_2)
\end{align}
Where $\alpha_1$ (resp. $\alpha_2$) is the hyperparameter that describes how much the rankings should redistribute utility on the user (resp. item) side.

\citet{do2021two} motivate the choice of additively separable welfare functions \eqref{eq:def-welf} by their usage in cardinal welfare economics \citep{dalton1920measurement,atkinson1970measurement,shorrocks1980class,cowell1988inequality}. Yet, their fairness criterion, which is based on the comparison of generalized Lorenz curves that we present in full detail in the next section, allows for other rankings than what can be generated by the family of additively separable welfare functions \eqref{eq:def-welf}. As we see in the next section, the generalized Gini welfare functions we optimize allows to generate \emph{every} ranking policy that \citet{do2021two} consider fair, and \emph{only} those. 



==> sections/old/old_gini.tex <==
\newpage
\section{Generalized Gini welfare functions} \label{sec:gini}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/lorenz_vs_generalized_lorenz.png}
    \caption{Lorenz curves (left) and Generalized Lorenz curves (right) of the distribution of income in Greece, in 2008 and 2012, taken from \citet{schneider2016changes} \nico{Placeholder}}
    \label{fig:lorenz}
\end{figure}

In this section we give the necessary background to understand the generalized Gini welfare functions, starting the exposition by the well-known Gini index of inequality \citep{gini1921measurement}.

\subsection{The Gini index and the Lorenz curve}

The Gini index \citep{gini1921measurement} is a well-known inequality measure used in welfare economics, in particular to quantify inequalities of wealth or income within a population \citep{chakravarty2009inequality}. Let $\bx\in\Re^n$ be a utility vector which contains the utility of $n$ individuals of a population of interest. The original definition is in terms of the Lorenz curve, which plots the fraction of total utility cumulated by fractions of the population ordered from the individual with minimum utility to the one with maximum utility. An example is given in Fig.~\ref{fig:lorenz}. The Gini index of $\bx$ is $1-2.A$ where $A$ is the area under the Lorenz curve of $\bx$. 

Formally, let $\bx\sort$ be the values of $\bx$ sorted in increasing order, i.e., $\bx_1\sort \leq ...\leq \bx_n\sort$ and let $\bxcum\in\Re^n$ be the cumulative sum of $\bx\sort$, i.e., $\bxcum_i = \bx_1\sort+...+\bx_i\sort$. The \emph{Lorenz curve} of $\bx$ is $i \mapsto \frac{\bxcum_i}{\norm{\bx}_1}$ (note that $\norm{\bx}_1=\bxcum_n$, so the end point of the curve is $1$), and the Gini index is
\begin{align}\label{eq:def:giniindex}
    \gini(\bx)= 1-\frac{2}{n\norm{\bx}_1}\sum_{i=1}^n \bxcum_i = 1-\frac{2}{n\norm{\bx}_1}\sum_{i=1}^n (n-i+1) \bu_i\sort.
\end{align}
If all the utility is owned by the best-off, then the Gini index is $1-\frac{2}{n} \xrightarrow[n\to\infty]{} 1$, while in a state of perfect equality (same utility for everyone), the Lorenz curve is a straight line from $(0,0)$ to $(1,1)$, in which case the Gini index is equal to $0$. Note that an alternative formula for the Gini index is \citep{yitzhaki2013more}:
\begin{align}
    \gini(\bx) = \frac{1}{n^2\bxm}\sum_{i=1}^n\sum_{j=1}^n |\bx_i-\bx_j| && \text{with~} \bxm=\frac{1}{n}\sum_{i=1}^n \bx_i.
\end{align}
which turns out to correspond to $\welfobjitem$ in \eqref{eq:def:eqexposure}.

A fundamental property of the Gini index is that it is decreasing with respect to the dominance of Lorenz curves. In words, if $\bx$ and $\bx'$ are such that the Lorenz curve of $\bx$ is always above that of $\bx'$ (i.e., $\forall i, \bxcum_i>\bxcum_i'$) then $\gini(\bx) < \gini(\bx')$. This is actually a fundamental property of all inequality measures \citep{cowell2000measurement}. This property follows the consensual part of the definition of inequality within a population, since if $\bx$ and $\bx'$ have the same mean, then, compared to $\bx'$, $\bx$ allocates more utility to the fractions of the population with less utility. The difference between inequality measures arise in the normative judgments they make when comparing $\bx$ and $\bx'$ when no Lorenz curve dominates each other, i.e., when the Lorenz curves intersect \citep{davies1995making,cowell2000measurement}.
% there is a book with Sen at least as a co-author with the quote that there is a consensus when Lorenz curves do not intersect

\subsection{Generalized Lorenz curves and welfare}

The measurement of inequality is concerned with the shape of the utility distribution, without regard to its mean. However, the mean is important when making decisions to maximize welfare, since otherwise we could choose solutions that reduce inequalities by making everyone worse-off. There is a duality in the domain of cardinal welfare economics between welfare functions, which give a value to policy decisions based on the resulting utility vector, and inequality measures \citep{atkinson1970measurement}. Up to the convention that welfare functions should be maximized and inequality measures minimized, their fundamental mathematical  property is the same up to the normalization of the Lorenz curve: welfare should be increasing with the dominance of \emph{unnormalized} Lorenz curves, called \emph{generalized Lorenz curves} and equal $i \mapsto \bxcum_i$ for utility vector $\bx$. Fig.~\ref{fig:lorenz} compares two utility vectors where the dominance of Lorenz and generalized Lorenz curves are inverted. From the point of view of cardinal welfare economics, the utility vector with dominant \emph{generalized} Lorenz curve should be preferred despite exhibiting more inequality, because every fraction of the population from the worse-off to the better-off receives more utility overall \citep{atkinson1970measurement,moulin2003fair}. As for inequality measures, the normative judgements underlying the specific choice of a welfare function aims at deciding, between utility vectors with intersecting generalized Lorenz curves, which ones are most suited to the problem at hand.

Generalized Gini welfare functions (GGFs) are a class of functions $\giniwelf{\bw}$ parameterized by a vector $\bw \in \reals^n$ of non-increasing positive weights, s.t. $\bw_1=1\geq\ldots\geq \bw_n\geq0$, and using the convention $\bw_{n+1}=0$. The GGFs are defined as:
\begin{align}\label{eq:def:ggf}
    \giniwelf{\bw}(\bx) = \sum_{i=1}^n (\bw_{i}-\bw_{i+1}) \bxcum_i = \sum_{i=1}^{n}\bw_i \bx_i\sort.
\end{align}
The right-hand side of \eqref{eq:def:ggf} writes $\giniwelf{\bw}$ as an ordered weighted averaging (OWA) operator \citep{yager1988ordered}. With non-increasing, non-negative $\bw$, it is well-known that OWA operators are concave \citep{fryer2005affirmative}. Moreover, if $\bw_i>0$ for all $i$, $\giniwelf{\bw}$ is increasing with respect to each input dimension \citep{fryer2005affirmative}. These two properties together ensure that when maximizing $\giniwelf{\bw}(\bx)$ over a set $\mathcal{X}\subset \Re_+^n$, all maximizers have non-dominated generalized Lorenz curves. \virginie{for someone who's not familiar with this literature, it may be a lot to digest.}

The choice of $\bw$ specifies the importance given to each fraction of the population. The following examples are well-known solutions: 
\begin{enumerate}
    \item $\bw = (1,1,\ldots, 1)$ corresponds to the standard utilitarian objective, maximizing the sum of utilities,
    \item $\bw \rightarrow (1,0,\ldots, 0)$ corresponds to the maximin egalitarian solution, giving all the weight to the worst-off individual,
    \item $\bw_i = \frac{n-i + 1}{n},$ is the welfare function of the Gini index.
\end{enumerate}

\subsection{Generating all non-Lorenz-dominated solutions}

When it comes to fairness in rankings, the fundamental property is that it can generate \emph{all} non-dominated Lorenz curves by properly setting the weights $\bw$. In this subsection we formalize this result borrowing the notion of Lorenz efficiency defined by \citet{do2021two}.

Let us first formalize the notion of \emph{Lorenz dominance}. Let $\bx$ and $\bx'$ two vectors in $\Re_+^n$. We say that $\bx$ weakly-Lorenz-dominates $\bx'$, denoted $\bx\lorenzw\bx'$, when the generalized Lorenz curve of $\bx$ is always at least equal to that of $\bx'$, i.e., $\bx\lorenzw\bx' \iff \forall i, \bxcum_i \geq \bxcum_i'$. We say that $\bx$ Lorenz-dominates $\bx'$, denoted $\bx\lorenz\bx'$ if $\bx\lorenzw\bx'$ and $\bx\neq\bx'$, i.e., if the generalized Lorenz curve of $\bx$ is strictly larger than that of $\bx'$ on at least one point. 

In the context of ranking and welfare functions, we have two groups of individuals: users and items. Since the utility of a user is not necessarily comparable to an item exposure, we consider their Lorenz curves separately. The criterion regarding the dominance of generalized Lorenz curves is extended to say that the utility vectors of interest should not be jointly dominated on users and items:
\begin{definition}[\citet{do2021two}]
A ranking policy $\rrk \in \rrkS$ is \emph{Lorenz-efficient} if there is no $\rrk' \in \rrkS$ such that either ($\bu(\rrk') \lorenzw\bu(\rrk)$ and $\bv(\rrk') \lorenz\bv(\rrk)$) or ($\bv(\rrk') \lorenzw\bv(\rrk)$ and $\bu(\rrk') \lorenz\bu(\rrk)$).
\end{definition}


let $\welfobj_{\lambda, \ubw, \ibw}(\rrk) = (1-\lambda)\giniwelf{\ubw}(\bu(\rrk) + \lambda \giniwelf{\ibw}(\bv(\rrk))$ the global welfare function \eqref{eq:welfobj} with $\welfobjuser = \giniwelf{\ubw}$ and $\welfobjitem=\giniwelf{\ibw}$. 


Formally. Let $\wS^1 = \{\ubw \in \reals^n: \,\ubw_1 = 1 \,\text{ and }\, \ubw_1 \geq \ldots \geq \ubw_n > 0\},$ let $\wS^2$ defined similarly in $\reals^m$, be the set of admissible weights of generalized Gini welfare functions. 
Let furthermore $\welfobj_{\lambda, \ubw, \ibw}(\rrk) = (1-\lambda)\giniwelf{\ubw}(\bu(\rrk) + \lambda \giniwelf{\ibw}(\bv(\rrk))$ the global welfare function \eqref{eq:welfobj} with $\welfobjuser = \giniwelf{\ubw}$ and $\welfobjitem=\giniwelf{\ibw}$.
Then:
\begin{proposition}\label{lem:all-lorenz} Let $\Theta=(0,1)\times\wS^1\times\wS^2$.
    \begin{enumerate}
        \item Let $(\lambda, \ubw, \ibw)\in\Theta$, and $\rrk^* \in \argmax\limits_{\rrk\in\rrkS}\welfobj_{\lambda, \ubw, \ibw}(\rrk)$. Then $\rrk^*$ is Lorenz-efficient. \virginie{actually, do we need strictly decreasing weights for this guarantee?}
        
        \item If $\rrk$ is Lorenz efficient, then there exists $(\iw,\ubw,\ibw) \in \Theta$ such that $\rrk\in\argmax_{\rrk \in \rrkS} \welfobj_{\lambda, \ubw, \ibw}(\rrk)$.
    \end{enumerate}
\end{proposition}
\begin{proof}
The proof uses standard results on convex multi-objective optimization from \citep{geoffrion1968proper,miettinen2012nonlinear}. The GGFs corresponds to the scalarization of the multi-objective problem of jointly maximizing the generalized Lorenz curves of users and items, which is a multi-objective problems with $n+m$ objectives (one objective for each point of the curve). We are optimizing over the convex set of stochastic ranking policies, and each objective function is concave because it corresponds to an OWA operator with non-increasing weight applied to utilities or exposures, which are linear functions of the ranking policy. The multi-objective problem is then concave, which means that all positive weighted sums of the objective are Pareto-efficient, and vice-versa: every Pareto-efficient solution is a solution of one positive weighted sum of the objectives.\nico{check if this is correct}. The result follows from the observation that the Lorenz-efficiency of $\rrk$ is equivalent to Pareto-efficiency of the set of points of the Lorenz-curves of users and items.
\end{proof}




==> sections/old/old_moreau.tex <==
\newpage
\section{The Moreau envelope of Genaralized Gini Welfare Functions} \label{sec:moreau-ggf}

\nico{this section could use a bit of elaboration on the technical challenge, with the clarification that you resolve these challenges by bringing pieces using work from different communities}

\nico{It is important that you want to use smoothing because you want to do FW because you do ranking. I'm not sure whethe it should come in this section or in the intro though}

The GGF is nondifferentiable because it requires to sort utilities. In order to use efficient gradient-based optimization methods, we smooth the GGF using its Moreau envelope \citep{moreau1962fonctions}. The contribution of this section is to show that the gradient of the Moreau envelope can be computed  in $O(n \log n).$

\paragraph{Notation} $\norm{\bz}_p = \left(\sum_{i=1}^n (z_i)^p \right)^{\frac{1}{p}}$ denotes the $\ell_p$ norm, and when unambiguous, we use $\|\cdot \|$ as a shorthand for $\|\cdot \|_2$. Given a linear map $\bu,$ $\norm{\bu}$ denotes the operator norm of $\bu,$ and $\bu^*$ is its adjoint. The Euclidean projection onto a convex $\mathcal{C}$ is denoted by $\proj_{\mathcal{C}}(\bz):= \argmin\limits_{\bc \in \mathcal{C}} \frac{1}{2} \norm{\bz - \bc}^2.$ $D_\mathcal{C} := \max\limits_{\bx, \bx' \in \mathcal{C}}\|\bx - \bx'\|$ is the diameter of $\mathcal{C}.$

\subsection{Definition and properties}

Let $\US \subseteq \reals^n$. Let us fix the OWA weights $\bw$ and denote the GGF $g(\bz) := g_{\bw}(\bz)$. We also introduce $h(\bz) = -g(\bz)$ 
to obtain a convex minimization problem: $\min\limits_{\bz \in \US} h(\bz)$. We notice that $h$ is $\|\bw\|$-Lipschitz continuous, and that: $~~h(\bz) = -\min\limits_{\sigma \in \permSn} \bwsigt \bz = \max\limits_{\sigma \in \permSn } -\bwsigt \bz.$

% We consider the smooth approximation\footnote{It is also equal to the Moreau envelope of $h$, by strong duality.} of $h$ from \citet{nesterov2005smooth}, defined as: 
% \begin{equation}
%     \hbeta(\bz) = \max_{\by \in \reals^n} \xdp{\bz}{\by} - h^*(\by) - \frac{\beta}{2}\|\by\|,
% \end{equation} for some smoothing parameter $\beta > 0$.  The proximal operator is defined as $\prox_{\phi}(\bz) = \argmin _{\bz' \in \mathcal{U}} \phi(\bz) + \frac{1}{2}\|\bz'-\bz\|^2.$


We consider the smooth approximation of $h$ given by its Moreau envelope\footnote{By the Fenchel duality theorem \citep{rockafellar2015convex}, it is also equal to the smoothing technique of \citet{nesterov2005smooth} with the Euclidean proximity function $\frac{1}{2} \norm{\cdot}^2$, which is the dual formulation of the Moreau envelope (see \citep[Sec. 4.3]{beck2012smoothing}).} , defined as:
\begin{align}
    h^\beta(\bz) = \min_{\bz' \in \US} h(\bz') + \frac{1}{2 \beta} \norm{\bz - \bz'}^2.
\end{align}

The literature on nonsmooth convex optimization often considers nonsmooth problems of the form $\min\limits_{P \in \rrkS} h(\bu(\rrk)),$ where $\rrkS$ be a convex set, let $\bu: \rrkS \mapsto \reals^n$ is a linear operator \cite{lan2013complexity,yurtsever2018conditional}. Denoting $f = h \circ u$ and $\fbeta = \hbeta \circ u,$ the following lemma states previously established results on the smoothness and approximation properties of the Moreau envelope (see e.g., \citep{yurtsever2018conditional,2020thekumparampil}). 
\begin{lemma}[Properties of the Moreau envelope]\label{lem:moreau} Let $\beta > 0.$
\begin{enumerate}
    \item $\fbeta$ is $\frac{\|\bu\|^2}{\beta}$-smooth and $\grad \fbeta(P) = \frac{1}{\beta} \bu^* (\bu(P) - \prox_{\beta h}(\bu(P)).$
    \item $\forall \bz,\, \hbeta(\bz) \leq h(\bz) \leq \hbeta(\bz) + \frac{\beta}{2}\|\bw\|^2$.
\end{enumerate}
\end{lemma}

The parameter $\beta$ controls the trade-off between the smoothness of $\hbeta$ and the quality of its approximation of $h.$ 

\subsection{Efficient computation of the gradient} \label{sec:isotonic}

We now present our main technical contribution, which is an efficient procedure for the computation of the Moreau envelope's gradient. The main challenge is the calculation of $\prox_{\beta h}(\bv)$. We show that in our case, $\prox_{\beta h}(\bv)$ can be computed efficiently using a reduction to isotonic regression.

For $\bz \in \reals^n$, let $\ph(\bz)$ denote the permutahedron induced by $\bz$, defined as the convex hull of all permutations of the vector $\bz$: $\,\ph(\bz) = \conv\{\bcsig : \sigma \in \permSn\}.\,$ Then $h$ can be written as the support function of the convex $\ph(\tbw)$, where $\tbw = -(w_n,...,w_1)$:
\begin{align*}
    h(\bz) = \max_{\sigma \in \permSn} -\bwsigt \bz = \sup_{\by \in \ph(\tbw)} \by^\intercal \bz.
\end{align*}
Then the conjugate of $h$ is known to be the indicator function of the convex $\ph(\tbw)$, and its proximal is the projection $\proj_{\ph(\tbw)}$ \citep{parikh2014proximal}. By Moreau decomposition, we get: $~\prox_{\beta h}(\bz) = \bz - \beta \proj_{\ph(\tbw)}\left(\nicefrac{\bz}{\beta}\right),$ and thus:
\begin{equation}
\begin{aligned}\label{eq:yt-proj}
    \grad \fbeta(P) = \bu^* \left(\proj_{\ph(\tbw)}\left(\nicefrac{\bu(P)}{\beta}\right)\right).
\end{aligned}
\end{equation}


Therefore, computing $\prox_{\beta h}$ and the $\yt$ of Proposition \ref{prop:fwgrad} boils down to a projection onto the permutahedron $\ph(\tbw)$. This projection was shown by several authors to be reducible to isotonic regression \citep{negrinho2014orbit,lim2016efficient,blondel2020fast}.

\begin{proposition}[Reduction to isotonic regression \citep{lim2016efficient,blondel2020fast}]\label{prop:isoto} Let $\sigma\in\permSn$ that sorts $\bz$ decreasingly, i.e. $z_{\sigma(1)} \geq \ldots \geq z_{\sigma(n)}.$
Let $\bx$ be a solution to isotonic regression on $\bzsig - \tbw$, i.e.
\begin{align}
    \bx = \argmin_{x'_1 \leq \ldots \leq x'_n} \frac{1}{2}\|\bx' - (\bzsig - \bw)\|^2
\end{align}
Then we have: $ \proj_{\ph(\tbw)}(\bz) = \bz + \xvector{x_{\sigma^{-1}}}.$
\end{proposition}


We use the Pool Adjacent Violators (\PAV) algorithm for isotonic regression, which was shown to output an exact solution in $O(n)$ iterations given a sorted input \cite{best2000minimizing}. Including the sorting of the input, the algorithm for computing $\nabla \fbeta(P)$ only costs $O(n \log n)$ time and $O(n)$ space. 

\nico{Maybe to clarify your contribution you could state the proposition in terms of the gradient of generalized Gini, and differ the other results to a proof of that.}

\nico{After the proof (or at the beginning of the section, where you explain the pieces you bring together, I think it's worthwhile to mention the relationship and differences with differentiable sorting and Blondel et. al, because it feels this is timely work and it (may) increase the perception that what you say here is not well-known.}

----

\begin{proposition}\label{prop:fwgrad}
Let $\uyt=\proj_{\ph({\utbw})}\left(\frac{\bu(\rrkt)}{\sm_t}\right)$ and $\iyt=\proj_{\ph({\itbw})}\left(\frac{\bv(\rrkt)}{\sm_t}\right).$ Let $\tempmuij = (1-\iw) \uyt_i \muij + \iw \iyt_j$. For all $i \in \intint{n},$ let $\tilde{\sigma}_i \in \topk(-\tilde{\mu}_i)$ and $\Qt_i$ a permutation matrix representing $\tilde{\sigma}_i$.
Then $\Qt \in \argmin\limits_{\rrk \in \rrkS} \xdp{\rrk}{\grad \fbetat(\rrkt)}.$
\end{proposition}

\begin{proof}
Using the expression of the gradient of the Moreau envelope derived in Proposition \ref{prop:grad-moreau}, eq. \eqref{eq:grad-moreau}, we have:\begin{align*}
    \grad \fbeta(P) = (1 - \iw) \, \bu^* (\proj_{\ph(\utbw)}\left(\nicefrac{\bu(P)}{\beta}\right)) + \iw \, \bv^* (\proj_{\ph(\itbw)}\left(\nicefrac{\bv(P)}{\beta}\right))
\end{align*}

By definition of $\uyt,\iyt$, for all $\rrk \in \rrkS$ we have: \begin{align*}
    \xdp{\rrk}{\grad \fbetat(P^{(t)}}) &= (1 - \iw) \xdp{\rrk}{\bu^* (\uyt)} + \iw \xdp{\rrk}{\bv^* (\iyt)}) \\
    &= (1 - \iw) \xdp{\bu(P)}{\uyt} + \iw \xdp{\bv(P)}{\iyt}\\
    &= (1 - \iw) \sum_{i=1}^n\sum_{j=1}^m  \uyt_i \muij  \rrk_{ij} \ew + \iw \sum_{j=1}^m \sum_{i=1}^n \iyt_j \rrk_{ij} \ew \\
    %&= \sum_{i=1}^n\sum_{j=1}^m  \left((1 - \iw) \uyt_i \mu_i^\intercal + \iw \iyt_j  \right) \rrk_{ij} \ew.
    &= \sum_{i=1}^n\sum_{j=1}^m  \tempmuij \rrk_{ij} \ew.
\end{align*}
The result follows from Lem. 3 of \citep{do2021two} and is a consequence of the rearrangement lemma \cite{hardy1952inequalities}: the optimal $\Qt \in \argmin\limits_{\rrk \in \rrkS} \xdp{\rrk}{\grad \fbetat(\rrkt)}$ is obtained by sorting $\tempmuij$ in increasing order (or equivalently, $-\tempmuij$ in decreasing order since we consider the minimization of $f=-F$).
\end{proof}


% \paragraph{Summary of step \eqref{eq:fw-step}} Using \eqref{eq:prox}, the vector $\yt$ of Proposition \ref{prop:fwgrad} simply writes as the projection
% \begin{equation}
% \begin{aligned}
%     \yt =  \proj_{\ph(\tbw)}\left(\frac{\bu(\rrkt)}{\sm_t}\right),
% \end{aligned}
% \end{equation}
% and is computed by the formula of Proposition \ref{prop:isoto} using the Pool Adjacent Violators algorithm. The solution of step \eqref{eq:fw-step} is then obtained as a $\topk(\yt_i\mu_i)$ for each user $i$. Our full algorithm is described in Alg. \ref{alg:full}, App. \ref{app:morealgo}.



==> sections/old/old_old_framework.tex <==
\section{Ranking with two-sided fairness [0.75p / 2.5p]} \label{sec:framework}
\nico{II would say ``ranking'' rather than ``rankings''}

We consider a recommendation scenario with $n$ users, and $m$ items, and $K$ recommendation slots. $\mu_{ij} \in [0,1]$ denotes the value of item $j$ for user $i$ (e.g, a ``liking'' probability), and we assume the values $\mu$ are given as input to the recommender system. 

The goal of the system is to produce a ranked list of items for each of the $n$ users. %Formally, for all $i \in \intint{n},$ the recommender system outputs $\sigma_i, $ a permutation of $\intint{m}$, such that $\sigma_i(j)$ is the rank of item $j$ in the list shown to user $i.$ 
Following previous work on fair rankings \citep[e.g.][]{singh2018fairness}, we consider stochastic rankings because they enable (a) the use of convex optimization techniques, and (b) redistribution of exposure, in contrast to deterministic rankings where the same items capture most attention \nico{I'm not sure the end of the sentence is clear}. A stochastic ranking for user $i$ is represented by a bistochastic matrix $\rrk_i \in \reals^{m\times m},$ where $\rrk_{ijk}$ is the probability that item $j$ is recommended to user $i$ at position $k.$ The recommender system outputs a global stochastic ranking $\rrk = (\rrk_i)_{i=1}^n$, and we denote the convex set of global stochastic rankings by $\rrkS$.\nico{IIRC, people were confused by the term "global ranking" that they interpret as "a single ranking for everybody".}

In line with previous work, we consider a position-based model with non-increasing weights $\ew \in \reals_+^m,$ where $\ew_k$ is the probability that a user examines the item at position $k.$ Since there are $K$ recommendation slots, we have $\ew_1 \geq \ldots \geq \ew_K$ and $\ew_k = 0$ for any $k > K.$ 

Since the recommender system impacts both user and items, we model this two-sided impact through two notions of utility. The user utility is defined as the expected performance of the ranking for the user in the position-based model, and the item utility is their average total exposure to users:
\begin{align*}
    \textit{User utility: }\, u_i(P) = \sum_{j=1}^m \mu_i^\intercal \rrk_{ij} \ew &&\textit{Item exposure: }\, v_j(P) = \sum_{i=1}^m\rrk_{ij} \ew
\end{align*}

The set of feasible utility profiles is $\US= \{(\bx, \by) \in \reals^n \times \reals^m \,:\, \exists \rrk \in \rrkS, \bx = \bu(\rrk) ~ \text{and} ~ \by = \bv(\rrk) \}.$ In cardinal welfare economics, generalized Lorenz curves allow to diagnose the wellbeing of a society, by depicted how utility is distributed among fractions of the population, ordered from worse-off to better-off \citep{shorrocks1980class}. Given a utility vector $\bz$, let $\bzsort$ be the vector of values of $\bz$ sorted increasing order, i.e., $\bzsort_1 \leq \ldots \leq \bzsort_n$, then the generalized Lorenz curve of $\bz$ is $(Z_i)_{i=1}^n$ where $Z_i = \bzsort_1+\ldots+\bzsort_i$. Following \citep{do2021two}, we assess fairness based on two partial orderings of the utility vectors:

\textbf{Pareto-dominance $\pareto$.} $\bz\pareto\bz'\iff (\forall i\in\intint{n}, \bz_i\geq z'_i$ and $\exists i\in\intint{n}, \bz_i> z'_i)$.

\textbf{Lorenz-dominance $\lorenz$.} Then $\bz\lorenz\bz' \iff \bzcum\pareto\bzcump$. $\lorenzw$ denotes non-strict Lorenz dominance, i.e., $\forall i, \bzcum_i\geq \bzcump_i$.

We consider fairness in rankings as Lorenz efficiency:
\begin{definition}[Lorenz efficiency, \citet{do2021two}]
A global ranking $\rrk \in \rrkS$ is \emph{Lorenz-efficient} if there is no $\rrk' \in \rrkS$ such that either ($\bu(\rrk') \lorenzw\bu(\rrk)$ and $\bv(\rrk') \lorenz\bv(\rrk)$) or ($\bv(\rrk') \lorenzw\bv(\rrk)$ and $\bu(\rrk') \lorenz\bu(\rrk)$).
\end{definition}
% \begin{definition}[Lorenz efficiency]
% A utility profile $(\bx,\by) \in \US$ is \emph{Lorenz-efficient} if there is no $(\bx', \by') \in \US$ such that either ($\bx' \lorenzw\bx$ and $\by' \lorenz\by$) or ($\by' \lorenzw\by $ and $\bx'\lorenz\bx$).
% \end{definition}

In other words, Lorenz efficiency means that the Lorenz curves of users and items should not be jointly dominated. It is thus a \emph{two-sided} fairness criterion which accounts for both users and items' interests. This criterion encodes Pareto \textbf{efficiency}, because Pareto dominance implies Lorenz dominance. It also encodes \textbf{equity} in the sense of \emph{Pigou-Dalton transfers}: at all levels of total utility, utility should be redistributed from better-off to worse-off.


\virginie{Motivation: a richer evaluation of fairness.}



==> sections/old/old_old_gini.tex <==
\newpage
\section{Generalized Gini Indices [1p / 3.5p]} \label{sec:gini}
\virginie{Figure \ref{fig:lorenz} should illustrate what a generalized Lorenz curve is and what GGI does. [idem tweet figure?]}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/lorenz-variety_tradeoffs-1sided.png}
    \caption{Blue: utilitarian, winner-take-all. Green: Equal item exposures. Red: Equal item exposures with better utility for the 25\% worse-off users. Orange: intermediate trade-off.\nico{Placeholder}}
    \label{fig:lorenz}
\end{figure}

\subsection{The Gini index}
The Gini index \citep{gini1921measurement} is a well-known inequality measure used in welfare economics, in particular to quantify inequalities of wealth or income within a population. It is computed as \citep{yitzhaki2013more}:
\begin{align}
    \gini(\bx) = \frac{1}{n^2\bxm}\sum_{i=1}^n\sum_{j=1}^n |\bx_i-\bx_j| && \text{with~} \bxm=\frac{1}{n}\sum_{i=1}^n \bx_i.
\end{align}
%  The reader is invited to read \citet{cowell2000measurement} for the theory of inequality measures in welfare economics and to \citet{chakravarty2009inequality} for an extensive survey of measures used in practice. 
Note that in addition to the Gini index being a well-known measure of inequality, the sum of absolute pairwise differences previously appeared routinely in papers on fairness of exposure \citep{singh2018fairness,morik2020controlling} as measures of ``unfairness'', even though these papers do not explicitly mention the relationship with the Gini index.

\subsection{The Lorenz curve}

The Gini index has many definitions, one of the most used being based on the Lorenz curve, which plots cumulative fractions of utility owned by individuals ordered from those with less utility (the worse-off) to those with highest utility (the better-off). Formally, let $\bx\sort$ be the values of $\bx$ sorted in increasing order, i.e., $\bx_1\sort \leq ...\leq \bx_n\sort$ and let $\bxcum\in\Re^n$ be the cumulative sum of $\bx\sort$, i.e., $\bxcum_i = \bx_1\sort+...+\bx_i\sort$. The \emph{Lorenz curve} of $\bx$ is $i/n \mapsto \frac{\bxcum_i}{\norm{\bx}_1}$ (note that $\norm{\bx}_1=\bxcum_n$, so the end point of the curve is $1$). Then the Gini index is equal to 1-2*A where $A$ is the area under the Lorenz curve:
\begin{align}
    \gini(\bx)= 1-\frac{2}{n\norm{\bx}_1}\sum_{i=1}^n \bxcum_i.
\end{align}
An example of Lorenz curve is given Fig.~\ref{fig:lorenz}. It provides the complete profile of how utility is distributed across the population. When there is perfect equality of utility, the lorenz curve is a straight line from $(0,0)$ to $(1,1)$, whereas the flatter the curve, the more the utility is concentrated on the better-off individuals. 

\subsection{The welfare function of the Gini index}

As elaborated by \citet{atkinson1970measurement}, when choosing an inequality measure, the underlying question are the implications for welfare: how does minimizing an inequality measure translates into collective decisions. The welfare function associated to the Gini index is the un-normalized value $\frac{1}{n}\sum_{i=1}^n \bxcum_i$. The normalization by $\frac{1}{n}$ is a matter of convention since the values of the welfare function do not matter in themselves. The important properties of the Welfare function depend on the decision you obtain by maximizing them.

The fundamental difference between the Gini coefficient and it's associated welfare function is the absence of normalization. As elaborated by \citet{atkinson1970measurement} and discussed in the context of fairness in ranking by \citet{do2021two}, inequality measures focus only on the shape of the distribution, not on its mean. This implies that it is possible to reduce inequalities by making everyone worse-off, which is undesirable. The absence of normalization in the Welfare function prevents this behavior. 

In the sequel, we call \emph{generalized} Lorenz curves the Lorenz curves without normalization, i.e. the curve $i/n \mapsto \bxcum_i$ \citep{shorrocks1983ranking}. It is convenient for the next subsection to rewrite the Gini welfare as the area under the generalized Lorenz curve, or equivalently as an ordered weighted average (OWA, \citep{yager1988ordered}):
\begin{align}\label{eq:giniowa}
    \welfgini(\bx) = \frac{1}{n}\sum_{i=1}^n \bxcum_i = \sum_{i=1}^n \frac{n-i+1}{n} \bx_i\sort.
\end{align}
This formula clarifies that the utility of the worse-off ($\bx_i\sort$ for small $i$) account for more than the utility of the better-off. Note that the right-hand side of the formula above is called an ordered weighted average because the weight associated to a coordinate in $\bx$ depends on its rank after sorting in increasing order. 



\subsection{Optimizing the generalized Lorenz curve}

Welfare functions and inequality measures alike define normative judgements on how \emph{more inequality} is desired. These values are often described in terms of redistribution or transfers from better-off to worse-off individuals in the population. The Gini index \eqref{eq:giniowa} gives equal weight to the cumulative share of each fraction of the population, in the sense that each point of the generalized Lorenz curve $\bxcum_i$ has equal weight \eqref{eq:giniowa} (which corresponds to giving more weight to worse-off individuals of the population, where the weight is a linear function of the rank, as shown by the weight $\frac{n-i+1}{n}$ assigned to $\bx_i\sort$). 

Since the generalized Lorenz curve uniquely characterizes the distribution of utility in the population \citep{shorrocks1983ranking}, a natural way to formulate normative judgements in terms of redistribution is by assigning weights to each point of the Lorenz curve. This family of welfare function is called Generalized Gini welfare Functions (GGFs, \citep{weymark1981generalized}), which can be written as an ordered weighted average of utilities. Given a vector $\bw$ of non-increasing positive weights, s.t. $\bw_1=1\geq\ldots\geq \bw_n\geq0$, and using the convention $\bw_{n+1}=0$, the GGFs are defined as:
\begin{align}
    g_{\bw}(\bx) = \sum_{i=1}^n (\bw_{i}-\bw_{i+1}) \bxcum_i = \sum_{i=1}^{n}\bw_j \bx_i\sort.
\end{align}
The fact that the weights $\bw$ are non-increasing imply that $\bw_{i}-\bw_{i+1}\geq 0$, and also that $\welfgini$ is concave \citep{yager1988ordered}. It is clear also that $g_{\bw}(\bx)$ is increasing with respect to each coordinate in $\bx$. This guarantees that maximizing $\welfgini$ generates solutions that are Pareto-optimal and that $\welfgini$ is monotonic with respect to the dominance of generalized Lorenz curves.




\subsection{Multi-Objective Optimization of Lorenz curves}

We consider a multi-objective optimization problem where the goal is to optimize each point of the generalized Lorenz curves of users and items, over the set of stochastic ranking tensors $\rrkS$: $\,
    \max\limits_{\rrk \in \rrkS}\, (U_1(P),\ldots, U_n(P), V_1(P),\ldots V_m(P)).$
    
For $(\iw, \ulw, \ilw) \in [0,1]\times \reals_+^n \times \reals_+^m$ s.t. $\,\sum_{i=1}^n \ulw_i = 1$ and $\sum_{j=1}^n \ilw_j = 1$, the weighted sum objective is: 
\begin{align}\label{eq:mainobj}
    \max_{\rrk \in \rrkS} \, \,\left\{ F(P) :=(1-\iw) \sum_{i=1}^{n}\ulw_i U_i(P) + \iw \sum_{j=1}^{m} \ilw_j V_j(P) \right \}.
\end{align}

The choice of $\ilw_j$ controls the degree of priority to the $\frac{j}{m}$-$\%$ worse-off items, and $\ulw_i$ is for the $\frac{i}{n}$-$\%$ worse-off users, while $\iw$ controls the relative weight of users and items. Overall, there are two ``big'' objectives, one for users and one for items, and many ``small'' objectives for each individual of either populations.

Given a vector $\bw$ of nonincreasing positive weights, s.t. $\bw_1=1\geq\ldots\geq \bw_m\geq0,$ let $g_{\bw}(\bz) = \sum_{j=1}^{m}\bw_j \bzsort_j$ for a utility vector $\bz \in \reals^m.$ In welfare economics, the OWAs $g_{\bw}(\bz) = \sum_{j=1}^{m}\bw_j \bzsort_j$ are known as \emph{Generalized Gini inequality indices} (GGIs) \citep{weymark1981generalized}. Denoting $\ubw_i = \sum_{l=i}^n \ulw_l\,$ and $\ibw_j = \sum_{l=j}^m \ilw_l\,$, the weighted sum objective is then a weighted sum of two GGIs, one for users and one for items: %ordered weighted averages (OWAs) of utilities with nonincreasing positive weights $\ubw$ and $\ilw$: _1 \geq \ldots \geq \ubw_n > 0 $, and $\ibw_1 \geq \ldots \geq \ibw_m > 0 $:
\begin{align}\label{eq:owaobj}
    &F(P) = G(\bx(P), \bv(P)) \\
    &\text {with }~G(\bx, \by) = (1- \iw) g_{\ubw}(\bx) + \iw g_{\ibw}(\by).
\end{align} 
% \begin{align}
%     F(P) := \iw \sum_{i=1}^{n}\ubw_i u_i\sort(P) + (1-\iw) \sum_{j=1}^{m}\ibw_j v_j\sort(P).
% \end{align}

Our goal is to maximize $F(P)$ which balances between a GGI for users and a GGI for items. The fact that the OWA weights are decreasing gives priority to the worse-off, and favors transfers from better-off to worse-off. The parameters of $F(P)$ allow to control the complex multi-dimensional trade-off between users and items' utilities. 


\virginie{Give some background on Generalized Gini. It is usually defined with $\sum_{i=1}^n w_i = 1$.}

Let $\wS^1 = \{\ubw \in \reals^n: \,\ubw_1 = 1 \,\text{ and }\, \ubw_1 \geq \ldots \geq \ubw_n > 0\},$ let $\wS^2$ defined similarly in $\reals^m$, and let $\Theta = [0,1] \times \wS^1 \times \wS^2.$ Formulations \eqref{eq:mainobj} and \eqref{eq:owaobj} are equivalent.\footnote{Indeed, for any $\bw$ s.t. $\bw_1 =1$ and $w_1 \geq \ldots \geq w_n > 0$, one can define $\lw_l = w_l - w_{l+1}$ for $1\leq l<n\,$ and $\lw_n = w_n$, so that $\lw \geq 0$ and $\sum_{i=1}^n \lw_i = 1$.}

Since $F(P)$ is a sum of OWAs with nonincreasing weights, it is concave in the utilities $(\bx(P), \bv(P))$. Since all points of the Lorenz curves $U_i(P)$ or $V_j(P)$ can also be written as OWAs with nonincreasing weights, they are concave too:

\begin{lemma}\label{lem:owa-concave}
$F$ is concave. Moreover, for all $i,j \in \intint{n} \times \intint{m}, P \mapsto U_i(P)$ and $P \mapsto V_j(P)$ are concave.
\end{lemma}

Problem \ref{eq:mainobj} is then a concave maximization problem, but it is nondifferentiable because of the sorting operation involved by the OWA of utilities.

% \subsection{Objective functions}

% Two-sided fairness with two Gini, one for users and one for items: $$F(P) = G(\bx(P), \bv(P))$$
% \begin{align*}
%     G(\bx, \by) = (1- \iw) g_{\ubw}(\bx) + \iw g_{\ibw}(\by)
% \end{align*}

% Item-side fairness with a trade-off between sum user utility and a Gini for items (i.e., $\ibw = (1,\ldots, 1)$):
% $$F(P) =  (1- \iw) \sum_{i=1}^n u_i(P) + \iw g_{\bw}(v(P)).$$

\subsection{Generating all Lorenz efficient solutions} 

We now show the main advantage of maximizing GGIs, which is that they allow to generate \emph{every} Lorenz efficient rankings.


First, any solution of $\max_{\rrk \in \rrkS} F(P)$ where the OWA weights are all positive and strictly decreasing are Lorenz efficient (because it is Pareto efficient in the Lorenz space). Second, since each objective function $U_i, V_j$ is concave in $P$ and since the solution space $\rrkS$ is convex, the converse is also true: 
\begin{proposition}\label{lem:all-lorenz} The GGI satisfies the following properties:
    \begin{enumerate}
        \item For any choice of $(\iw,\ubw,\ibw) \in \Theta$ such that $\ubw_1 > \ldots > \ubw_n > 0$ and $\ibw_1 > \ldots > \ibw_m > 0$ , if $P \in \argmax_{\rrk \in \rrkS} F(P)$, then $P$ is Lorenz efficient.
        \item If $P$ is Lorenz efficient, then there exists $(\iw,\ubw,\ibw) \in \Theta$ such that $P$ is a solution of $\max_{\rrk \in \rrkS} F_{\bw}(P)$.
    \end{enumerate}
\end{proposition}

The proof uses standard results on convex multi-objective optimization from \citep{geoffrion1968proper,miettinen2012nonlinear}. \nico{I think it is fairly important to insist on what properties of the problem make GGI equivalent to multi-objective optim. of the Lorenz curve. Maybe we should say that in the language of multi-objective optimization, GGIs correspond to the scalarization of the multi-objective problem. Scalarization allows to obtain all Pareto-efficient solutions if the multi-objective problem is convex. In our case, Pareto for Lorenz curves means Lorenz efficient, and we're convex because of the linearity of user utility/item exposure and the relaxation to stochastic rankings} Note that in the second bullet point, the OWA weights only need to be non-increasing. The GGI formulation covers the whole Lorenz set and thus allows to choose among a large variety of fair trade-offs by setting the weights $(\iw,\ubw,\ibw)$. The choice of fair trade-off depends on which fraction of the population the decision-maker aims to prioritize. Extreme choices of $(\iw,\ubw,\ibw)$ lead to well-known solutions: 
\begin{enumerate}
    \item $\iw=0, \ubw = (1,1,\ldots, 1)$ corresponds to the standard utilitarian ranking (obtained by sorting by decreasing $\mu_{ij}$ for each user $i$),
    \item $g_{\bw}(\bz)$ with $\bw \rightarrow (1,0,\ldots, 0)$ leads to the maxmin egalitarian solution.
    \item $g_{\bw}(\bz)$ with $\bw_j = \frac{n-j + 1}{n},$ is the classic Gini index.
\end{enumerate}

% The special case of a trade-off between total user utility and item-side fairness is also interesting to consider, by setting $\ubw = (1, \ldots, 1)$ and writing $\ibw = \bw$: 
% \begin{align}\label{eq:item-ggi}
%     F(P) =  (1- \iw) \sum_{i=1}^n u_i(P) + \iw g_{\bw}(\bv(P)).
% \end{align}

\subsection{WIP: some references}

Gini index was defined in \citep{gini1921measurement}. 

elements of discussion: 
\begin{itemize}
    \item \citet[Section 1]{atkinson1970measurement} for a discussion on the task of ranking distributions -- this paper is one of the first to make the link between measurement of inequality and schur concavity \citep{shorrocks1983ranking,bishop1991rank}. This paper also proposes Atkinson indices, which defines an inequality measure from a welfare function (see Section 5 and end of Section 4).
    
    The question as formulated by Atkinson and Dalton is that of the welfare impications of the choice of the inequality measure. This is the way to describe and justify the value judgements underlying the distributive criterion we want to optimize.
    
    
    \item About additive separability: \citet[Section 4]{atkinson1970measurement} \emph{The social welfare function considered here is assumed to be of the form (1) that we have been discussing throughout; that is, it is symmetric andadditively separable in individual incomes-although this is, of course, restrictive.} As explained in \citep[Section 1]{atkinson1970measurement}, the focus on additive separability of Atkinson follows Dalton's stance \citep{dalton1920measurement}, see \citet{atkinson2015unveiling} for a more recent discussion of Dalton's work.
    
    \citep{sheshinski1972relation} describes the welfare function associated to Gini. It's not additively separable but there is no discussion on whether it's desirable or undesirable \emph{But an additive welfare function has, of course, no particular sigticance. } \citep{sheshinski1972relation}. 
    
    Additive separability follows from the axiom of \emph{independence of unconcerned agents} of welfare functions \citep{moulin2003fair}. 
    \item more about decomposability: \citet{shorrocks1980class} defines the group-decomposable measures. 
    
    \item \citet[Section 4]{atkinson1970measurement} for discussion on mean-normalization, and advocation for strict concavity (which is not satisfied by measures such as interquantile range or focus on specific points of the Lorenz curve. 
    
    Also see point (c) of the conclusion of comparing the five standard inequality measures (including variance, stdev and Gini): \emph{The coefficient of variation attaches equal weight to transfers at
different income levels, the Gini coefficient attaches more weight to transfers affecting middle income classes and the standard deviation
weights transfers at the lower end more heavily.}. Note that a closer inspection of the explanation reveals that the argument regarding Gini is that the effect of (small) transfers (i.e., from an individual with utility $u$ to an inidivudal with utility $u-\epsilon$ are proportional (in the limit of a continuous distribution) to the density of the population at level of income $u$, so this interpretation of Gini as 'more affected by middle class' defines 'middle class' as where the density of the population is higher. Also note that Atkinson's argument here is about a transfer from people who have very close utility, not from richest to poorest.

\end{itemize}


Inequality indices defined as OWA operators (my source here is \citet{aristondo2013}, cite \citep{chakravarty2009inequality} for a review on inequality measures) \emph{The Bonferroni and De Vergottini indices are two other classical inequality indices that are recently receiving growing attention, see for instance Nygard and Sandstrom [41], Giorgi [28,29], Tarsitano [48], Giorgi and Mondani
[31], Giorgi and Crescenzi [30], Chakravarty and Muliere [13], Piesch [42], Chakravarty [11] and B´arcena and Imedio [3]. Similarly to the Gini index, they also permit negative incomes.}:
\begin{itemize}
    \item Bonferroni index with implicit weighting $w_i=\sum_{j=n-i+1}^n \frac{1}{j}$. De Vergottini is a dual of Bonferroni and they are equal up to affine transforms; they are equivalent as far as this work is concerned.
    \item quantile ratios \citet{burkhauser2009using} is a well-cited example of using 10\%/90\% quantiles of utilities to the measurement of inequality. \citet{prendergast2018simple} provide a complete discussion of using ratios of symmetric quantiles and its associated curve. 
    \item \citet{neves2019not} is another paper where they mention quantile ratios (not necessarily symmetric) as standard measures of inequality. 
\end{itemize}

Other inequality indices that are not easily written as OWA operators:
\begin{itemize}
    \item Theil, Atkinson and aditively separable measures which have easy-to-write welfare functions -> optimize them similarly to \citet{do2021two}. There are still problems of derivatives at 0, but in practice it may not be that bad
    \item Zenga index \citep{zenga2007inequality}, which may have better properties than Gini regarding how transfers from rich to poor are counted \citep{greselin2020social}.
\end{itemize}

==> sections/old/trash_introduction.tex <==
\section{Introduction [1p/1p]} \label{sec:intro}

Generalized Lorenz curves are studied in welfare economics to assess the wellbeing of a population in distributive terms, by representing the fraction of utility detained by the worse and better-off quantiles of the population. They were recently introduced for fairness assessments in recommender systems, where both users and items are impacted by the recommendations. In this paper,
we propose to generate fair rankings by maximizing each point of the generalized Lorenz curves of users and items. This multi-objective problem is equivalent to maximizing generalized Gini indices (GGI) \citep{weymark1981generalized}, a class of ordered weighted averages (OWAs). Compared to existing approaches based on additive concave welfare functions or equality constraints, GGIs provide a more general approach with better control on which fraction of the population should be prioritized.

Optimizing GGIs for rankings poses two major challenges: first, the OWA operator is non-differentiable because it involves sorting utilities, which prevents from using efficient gradient-based optimization schemes. Second, the optimization is over the space of three-dimensional global rankings, which contains a prohibitively large number of parameters. We show how to leverage nonsmooth Frank-Wolfe algorithms to efficiently compute fair rankings, for both static inference setting and online learning-to-rank. \nico{clarify the algorithmic contribution here}


\virginie{clarify this: The algorithmic contribution is a computationally efficient method for the calculation of the gradient of the Moreau envelope of convex OWAs.}

\paragraph{Notation} Given an integer $n \in \mathbb{N},$ $\intint{n} := \{1,\ldots,n\}\,$, and $\permSn$ denotes the set of permutations of $\intint{n}.$ Given $\bz \in \reals^n$, $\argsort\sort(\bz) = \{\sigma\in \permSn: z_{\sigma(1)} \leq\ldots\leq z_{\sigma(n)}\}$ sorts $\bz$ in increasing order, and $\argsort\descsort$ decreasingly. Let $\topk(\bz) = \{ \sigma \in \permSn: z_{\sigma(1)}\geq \ldots \geq z_{\sigma(K)}\}$.
Given a vector $\bz\in\Re^n$, let $\bzsort$ be the vector of values of $\bz$ sorted increasing order, i.e., $\bzsort_1 \leq \ldots \leq \bzsort_n$, then the generalized Lorenz curve of $\bz$ is $\bzcum = (\bzcum_i)_{i=1}^n$ where $\bzcum_i = \bzsort_1+\ldots+\bzsort_i$. 

\nico{maybe clean or remove this notation part -- what do we really need?}\nico{should we define the notation for the dot product?}\nico{We should probably say that vectors are in bold and we "de-bold" when we take the subscript}
